Stellar granulation and interferometry

Stars are not smooth. Their photosphere is covered by a granulation pattern associated with the heat transport by convection. The convection-related surface structures have different size, depth, and temporal variations with respect to the stellar type. The related activity (in addition to other phenomena such as magnetic spots, rotation, dust, etc.) potentially causes bias in stellar parameters determination, radial velocity, chemical abundances determinations, and exoplanet transit detections. The role of long-baseline interferometric observations in this astrophysical context is crucial to characterize the stellar surface dynamics and correct the potential biases. In this Chapter, we present how the granulation pattern is expected for different kind of stellar types ranging from main sequence to extremely evolved stars of different masses and how interferometric techniques help to study their photospheric dynamics.

==> biblio.tex <==
@ARTICLE{1801RSPT...91..265H,
   author = {{Herschel}, W.},
    title = "{Observations Tending to Investigate the Nature of the Sun, in Order to Find the Causes or Symptoms of Its Variable Emission of Light and Heat; With Remarks on the Use That May Possibly Be Drawn from Solar Observations}",
  journal = {Royal Society of London Philosophical Transactions Series I},
     year = 1801,
   volume = 91,
    pages = {265-318},
   adsurl = {http://adsabs.harvard.edu/abs/1801RSPT...91..265H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...610L.137C,
   author = {{Carlsson}, M. and {Stein}, R.~F. and {Nordlund}, {\AA}. and 
	{Scharmer}, G.~B.},
    title = "{Observational Manifestations of Solar Magnetoconvection: Center-to-Limb Variation}",
  journal = {\apjl},
   eprint = {astro-ph/0406160},
 keywords = {Convection, Magnetic Fields, Magnetohydrodynamics: MHD, Sun: Faculae, Plages, Sun: Photosphere},
     year = 2004,
    month = aug,
   volume = 610,
    pages = {L137-L140},
      doi = {10.1086/423305},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...610L.137C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...769...18T,
   author = {{Trampedach}, R. and {Asplund}, M. and {Collet}, R. and {Nordlund}, {\AA}. and 
	{Stein}, R.~F.},
    title = "{A Grid of Three-dimensional Stellar Atmosphere Models of Solar Metallicity. I. General Properties, Granulation, and Atmospheric Expansion}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1303.1780},
 primaryClass = "astro-ph.SR",
 keywords = {convection, stars: atmospheres, stars: interiors, stars: late-type },
     year = 2013,
    month = may,
   volume = 769,
      eid = {18},
    pages = {18},
      doi = {10.1088/0004-637X/769/1/18},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...769...18T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005A&A...431..773R,
   author = {{Richichi}, A. and {Percheron}, I. and {Khristoforova}, M.},
    title = "{CHARM2: An updated Catalog of High Angular Resolution Measurements}",
  journal = {\aap},
 keywords = {techniques: high angular resolution, techniques: interferometric, catalogs, occultations, stars: binaries: general, stars: fundamental parameters},
     year = 2005,
    month = feb,
   volume = 431,
    pages = {773-777},
      doi = {10.1051/0004-6361:20042039},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...431..773R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005LRSP....2....8B,
   author = {{Berdyugina}, S.~V.},
    title = "{Starspots: A Key to the Stellar Dynamo}",
  journal = {Living Reviews in Solar Physics},
 keywords = {starspots, sunspots, stellar magnetic fields, stellar cycles, dynamo, differential rotation, Doppler imaging},
     year = 2005,
    month = dec,
   volume = 2,
    pages = {8},
      doi = {10.12942/lrsp-2005-8},
   adsurl = {http://adsabs.harvard.edu/abs/2005LRSP....2....8B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2009A&ARv..17..251S,
   author = {{Strassmeier}, K.~G.},
    title = "{Starspots}",
  journal = {\aapr},
 keywords = {Starspots, Stars: activity, Stars: imaging, Sunspots, Magnetic fields, Techniques: polarimetric, Stars: rotation, Exoplanets},
     year = 2009,
    month = sep,
   volume = 17,
    pages = {251-308},
      doi = {10.1007/s00159-009-0020-6},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26ARv..17..251S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2014AAS...22320202A,
   author = {{Armstrong}, J.~T. and {Restaino}, S.~R. and {Clark}, J.~H. and 
	{Schmitt}, H.~R. and {Baines}, E.~K. and {Hutter}, D.~J. and 
	{Benson}, J.~A. and {Zavala}, R.~T. and {Shankland}, P.~D. and 
	{van Belle}, G. and {Jorgensen}, A.~M.},
    title = "{Progress in the expansion of the Navy Precision Optical Interferometer}",
booktitle = {American Astronomical Society Meeting Abstracts},
     year = 2014,
   series = {American Astronomical Society Meeting Abstracts},
   volume = 223,
    month = jan,
    pages = {#202.02},
   adsurl = {http://adsabs.harvard.edu/abs/2014AAS...22320202A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007A&A...473..983D,
   author = {{Desort}, M. and {Lagrange}, A.-M. and {Galland}, F. and {Udry}, S. and 
	{Mayor}, M.},
    title = "{Search for exoplanets with the radial-velocity technique: quantitative diagnostics of stellar activity}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0708.4338},
 keywords = {techniques: radial velocities, stars: early-type, stars: planetary systems, stars: starspots, stars: activity},
     year = 2007,
    month = oct,
   volume = 473,
    pages = {983-993},
      doi = {10.1051/0004-6361:20078144},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...473..983D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...743...61S,
   author = {{Sanchis-Ojeda}, R. and {Winn}, J.~N.},
    title = "{Starspots, Spin-Orbit Misalignment, and Active Latitudes in the HAT-P-11 Exoplanetary System}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1107.2920},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems, stars: activity, stars: individual: HAT-P-11, stars: rotation, starspots},
     year = 2011,
    month = dec,
   volume = 743,
      eid = {61},
    pages = {61},
      doi = {10.1088/0004-637X/743/1/61},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743...61S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997ApJ...485..319S,
   author = {{Saar}, S.~H. and {Donahue}, R.~A.},
    title = "{Activity-related Radial Velocity Variation in Cool Stars}",
  journal = {\apj},
 keywords = {CONVECTION, STARS: PLANETARY SYSTEMS, STARS: ACTIVITY, STARS: LATE-TYPE, TECHNIQUES: RADIAL VELOCITIES},
     year = 1997,
    month = aug,
   volume = 485,
    pages = {319},
      doi = {10.1086/304392},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...485..319S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004AJ....127.3579P,
   author = {{Paulson}, D.~B. and {Cochran}, W.~D. and {Hatzes}, A.~P.},
    title = "{Searching for Planets in the Hyades. V. Limits on Planet Detection in the Presence of Stellar Activity}",
  journal = {\aj},
   eprint = {astro-ph/0402569},
 keywords = {Galaxy: Open Clusters and Associations: Individual: Name: Hyades, Stars: Activity, Techniques: Radial Velocities},
     year = 2004,
    month = jun,
   volume = 127,
    pages = {3579-3586},
      doi = {10.1086/420710},
   adsurl = {http://adsabs.harvard.edu/abs/2004AJ....127.3579P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1998ApJ...498L.153S,
   author = {{Saar}, S.~H. and {Butler}, R.~P. and {Marcy}, G.~W.},
    title = "{Magnetic Activity-related Radial Velocity Variations in Cool Stars: First Results from the Lick Extrasolar Planet Survey}",
  journal = {\apjl},
 keywords = {STARS: PLANETARY SYSTEMS, STARS: ACTIVITY, CONVECTION, STARS: SPOTS, STARS: LATE-TYPE, TECHNIQUES: RADIAL VELOCITIES},
     year = 1998,
    month = may,
   volume = 498,
    pages = {L153},
      doi = {10.1086/311325},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...498L.153S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997Natur.385..795G,
   author = {{Gray}, D.~F.},
    title = "{Absence of a planetary signature in the spectra of the star 51 Pegasi}",
  journal = {\nat},
     year = 1997,
    month = feb,
   volume = 385,
    pages = {795-796},
      doi = {10.1038/385795a0},
   adsurl = {http://adsabs.harvard.edu/abs/1997Natur.385..795G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJS..117..563B,
   author = {{Brown}, T.~M. and {Kotak}, R. and {Horner}, S.~D. and {Kennelly}, E.~J. and 
	{Korzennik}, S. and {Nisenson}, P. and {Noyes}, R.~W.},
    title = "{Exoplanets or Dynamic Atmospheres? The Radial Velocity and Line Shape Variations of 51 Pegasi and tau Bootis}",
  journal = {\apjs},
   eprint = {astro-ph/9801166},
 keywords = {LINE: PROFILES, STARS: INDIVIDUAL CONSTELLATION NAME: TAU BOOTIS, STARS: INDIVIDUAL CONSTELLATION NAME: 51 PEGASI, STARS: PLANETARY SYSTEMS, STARS: OSCILLATIONS},
     year = 1998,
    month = jul,
   volume = 117,
    pages = {563},
      doi = {10.1086/313123},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJS..117..563B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995Natur.378..355M,
   author = {{Mayor}, M. and {Queloz}, D.},
    title = "{A Jupiter-mass companion to a solar-type star}",
  journal = {\nat},
     year = 1995,
    month = nov,
   volume = 378,
    pages = {355-359},
      doi = {10.1038/378355a0},
   adsurl = {http://adsabs.harvard.edu/abs/1995Natur.378..355M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2013MNRAS.435.2501L,
   author = {{Lachaume}, R. and {Berger}, J.-P.},
    title = "{Bandwidth smearing in infrared long-baseline interferometry. Application to stellar companion search in fringe-scanning mode}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1307.2907},
 primaryClass = "astro-ph.IM",
 keywords = {atmospheric effects, instrumentation: interferometers, methods: analytical, methods: data analysis},
     year = 2013,
    month = nov,
   volume = 435,
    pages = {2501-2519},
      doi = {10.1093/mnras/stt1462},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.435.2501L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...633..465S,
   author = {{Sato}, B. and {Fischer}, D.~A. and {Henry}, G.~W. and {Laughlin}, G. and 
	{Butler}, R.~P. and {Marcy}, G.~W. and {Vogt}, S.~S. and {Bodenheimer}, P. and 
	{Ida}, S. and {Toyota}, E. and {Wolf}, A. and {Valenti}, J.~A. and 
	{Boyd}, L.~J. and {Johnson}, J.~A. and {Wright}, J.~T. and {Ammons}, M. and 
	{Robinson}, S. and {Strader}, J. and {McCarthy}, C. and {Tah}, K.~L. and 
	{Minniti}, D.},
    title = "{The N2K Consortium. II. A Transiting Hot Saturn around HD 149026 with a Large Dense Core}",
  journal = {\apj},
   eprint = {astro-ph/0507009},
 keywords = {Stars: Planetary Systems, stars: individual (HD 149026)},
     year = 2005,
    month = nov,
   volume = 633,
    pages = {465-473},
      doi = {10.1086/449306},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...633..465S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011Natur.470...53L,
   author = {{Lissauer}, J.~J. and {Fabrycky}, D.~C. and {Ford}, E.~B. and 
	{Borucki}, W.~J. and {Fressin}, F. and {Marcy}, G.~W. and {Orosz}, J.~A. and 
	{Rowe}, J.~F. and {Torres}, G. and {Welsh}, W.~F. and {Batalha}, N.~M. and 
	{Bryson}, S.~T. and {Buchhave}, L.~A. and {Caldwell}, D.~A. and 
	{Carter}, J.~A. and {Charbonneau}, D. and {Christiansen}, J.~L. and 
	{Cochran}, W.~D. and {Desert}, J.-M. and {Dunham}, E.~W. and 
	{Fanelli}, M.~N. and {Fortney}, J.~J. and {Gautier}, III, T.~N. and 
	{Geary}, J.~C. and {Gilliland}, R.~L. and {Haas}, M.~R. and 
	{Hall}, J.~R. and {Holman}, M.~J. and {Koch}, D.~G. and {Latham}, D.~W. and 
	{Lopez}, E. and {McCauliff}, S. and {Miller}, N. and {Morehead}, R.~C. and 
	{Quintana}, E.~V. and {Ragozzine}, D. and {Sasselov}, D. and 
	{Short}, D.~R. and {Steffen}, J.~H.},
    title = "{A closely packed system of low-mass, low-density planets transiting Kepler-11}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1102.0291},
 primaryClass = "astro-ph.EP",
     year = 2011,
    month = feb,
   volume = 470,
    pages = {53-58},
      doi = {10.1038/nature09760},
   adsurl = {http://adsabs.harvard.edu/abs/2011Natur.470...53L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...528A..97T,
   author = {{Tingley}, B. and {Endl}, M. and {Gazzano}, J.-C. and {Alonso}, R. and 
	{Mazeh}, T. and {Jorda}, L. and {Aigrain}, S. and {Almenara}, J.-M. and 
	{Auvergne}, M. and {Baglin}, A. and {Barge}, P. and {Bonomo}, A.~S. and 
	{Bord{\'e}}, P. and {Bouchy}, F. and {Bruntt}, H. and {Cabrera}, J. and 
	{Carpano}, S. and {Carone}, L. and {Cochran}, W.~D. and {Csizmadia}, S. and 
	{Deleuil}, M. and {Deeg}, H.~J. and {Dvorak}, R. and {Erikson}, A. and 
	{Ferraz-Mello}, S. and {Fridlund}, M. and {Gandolfi}, D. and 
	{Gillon}, M. and {Guenther}, E.~W. and {Guillot}, T. and {Hatzes}, A. and 
	{H{\'e}brard}, G. and {L{\'e}ger}, A. and {Llebaria}, A. and 
	{Lammer}, H. and {Lovis}, C. and {MacQueen}, P.~J. and {Moutou}, C. and 
	{Ollivier}, M. and {Ofir}, A. and {P{\"a}tzold}, M. and {Pepe}, F. and 
	{Queloz}, D. and {Rauer}, H. and {Rouan}, D. and {Samuel}, B. and 
	{Schneider}, J. and {Shporer}, A. and {Wuchterl}, G.},
    title = "{Transiting exoplanets from the CoRoT space mission. XVI. CoRoT-14b: an unusually dense very hot Jupiter}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1101.1899},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems, techniques: photometric, techniques: radial velocities, techniques: spectroscopic},
     year = 2011,
    month = apr,
   volume = 528,
      eid = {A97},
    pages = {A97},
      doi = {10.1051/0004-6361/201015480},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...528A..97T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2012A&A...541A..89L,
   author = {{Le Bouquin}, J.-B. and {Absil}, O.},
    title = "{On the sensitivity of closure phases to faint companions in optical long baseline interferometry}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1204.3721},
 primaryClass = "astro-ph.IM",
 keywords = {techniques: interferometric, binaries: close, stars: low-mass, brown dwarfs, planets and satellites: detection},
     year = 2012,
    month = may,
   volume = 541,
      eid = {A89},
    pages = {A89},
      doi = {10.1051/0004-6361/201117891},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...541A..89L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...535A..67L,
   author = {{Le Bouquin}, J.-B. and {Berger}, J.-P. and {Lazareff}, B. and 
	{Zins}, G. and {Haguenauer}, P. and {Jocou}, L. and {Kern}, P. and 
	{Millan-Gabet}, R. and {Traub}, W. and {Absil}, O. and {Augereau}, J.-C. and 
	{Benisty}, M. and {Blind}, N. and {Bonfils}, X. and {Bourget}, P. and 
	{Delboulbe}, A. and {Feautrier}, P. and {Germain}, M. and {Gitton}, P. and 
	{Gillier}, D. and {Kiekebusch}, M. and {Kluska}, J. and {Knudstrup}, J. and 
	{Labeye}, P. and {Lizon}, J.-L. and {Monin}, J.-L. and {Magnard}, Y. and 
	{Malbet}, F. and {Maurel}, D. and {M{\'e}nard}, F. and {Micallef}, M. and 
	{Michaud}, L. and {Montagnier}, G. and {Morel}, S. and {Moulin}, T. and 
	{Perraut}, K. and {Popovic}, D. and {Rabou}, P. and {Rochat}, S. and 
	{Rojas}, C. and {Roussel}, F. and {Roux}, A. and {Stadler}, E. and 
	{Stefl}, S. and {Tatulli}, E. and {Ventura}, N.},
    title = "{PIONIER: a 4-telescope visitor instrument at VLTI}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1109.1918},
 primaryClass = "astro-ph.IM",
 keywords = {instrumentation: interferometers, techniques: interferometric, techniques: high angular resolution, instrumentation: high angular resolution},
     year = 2011,
    month = nov,
   volume = 535,
      eid = {A67},
    pages = {A67},
      doi = {10.1051/0004-6361/201117586},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...535A..67L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...535A..68A,
   author = {{Absil}, O. and {Le Bouquin}, J.-B. and {Berger}, J.-P. and 
	{Lagrange}, A.-M. and {Chauvin}, G. and {Lazareff}, B. and {Zins}, G. and 
	{Haguenauer}, P. and {Jocou}, L. and {Kern}, P. and {Millan-Gabet}, R. and 
	{Rochat}, S. and {Traub}, W.},
    title = "{Searching for faint companions with VLTI/PIONIER. I. Method and first results}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.1178},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: interferometric, binaries: close, stars: low mass, brown dwarfs, planetary systems},
     year = 2011,
    month = nov,
   volume = 535,
      eid = {A68},
    pages = {A68},
      doi = {10.1051/0004-6361/201117719},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...535A..68A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2010SPIE.7734E..37Z,
   author = {{Zhao}, M. and {Monnier}, J.~D. and {Che}, X. and {ten Brummelaar}, T. and 
	{Pedretti}, E. and {Thureau}, N.~D.},
    title = "{MIRC closure phase studies for high precision measurements}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2010,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 7734,
    month = jul,
      eid = {77341A},
      doi = {10.1117/12.857538},
   adsurl = {http://adsabs.harvard.edu/abs/2010SPIE.7734E..37Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011PASP..123..964Z,
   author = {{Zhao}, M. and {Monnier}, J.~D. and {Che}, X. and {Pedretti}, E. and 
	{Thureau}, N. and {Schaefer}, G. and {ten Brummelaar}, T. and 
	{M{\'e}rand}, A. and {Ridgway}, S.~T. and {McAlister}, H. and 
	{Turner}, N. and {Sturmann}, J. and {Sturmann}, L. and {Goldfinger}, P.~J. and 
	{Farrington}, C.},
    title = "{Toward Direct Detection of Hot Jupiters with Precision Closure Phase: Calibration Studies and First Results from the CHARA Array}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1109.5183},
 primaryClass = "astro-ph.EP",
     year = 2011,
    month = aug,
   volume = 123,
    pages = {964-975},
      doi = {10.1086/661762},
   adsurl = {http://adsabs.harvard.edu/abs/2011PASP..123..964Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2012AAS...21944613G,
   author = {{Ghasempour}, A. and {Muterspaugh}, M. and {Hutter}, D. and 
	{Monnier}, J. and {Armstrong}, T. and {Benson}, J. and {Mozurkewich}, D. and 
	{Williamson}, M. and {Fall}, S. and {Harrison}, C. and {Sergeyous}, C.
	},
    title = "{VISION: The Next Generation Science Camera for the Navy Optical Interferometer}",
booktitle = {American Astronomical Society Meeting Abstracts \#219},
     year = 2012,
   series = {American Astronomical Society Meeting Abstracts},
   volume = 219,
    month = jan,
    pages = {#446.13},
   adsurl = {http://adsabs.harvard.edu/abs/2012AAS...21944613G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012POBeo..91..129L,
   author = {{Lopez}, B.},
    title = "{Perspective of the Interferometric MATISSE Instrument at the VLTI}",
  journal = {Publications de l'Observatoire Astronomique de Beograd},
     year = 2012,
    month = dec,
   volume = 91,
    pages = {129-139},
   adsurl = {http://adsabs.harvard.edu/abs/2012POBeo..91..129L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...520L...2A,
   author = {{Absil}, O. and {Le Bouquin}, J.-B. and {Lebreton}, J. and {Augereau}, J.-C. and 
	{Benisty}, M. and {Chauvin}, G. and {Hanot}, C. and {M{\'e}rand}, A. and 
	{Montagnier}, G.},
    title = "{Deep near-infrared interferometric search for low-mass companions around {$\beta$} Pictoris}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1009.1245},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: {$\beta$} Pic, planets and satellites: detection, techniques: interferometric, planetary systems, stars: individual: {$\beta$} Pic},
     year = 2010,
    month = sep,
   volume = 520,
      eid = {L2},
    pages = {L2},
      doi = {10.1051/0004-6361/201015156},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...520L...2A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2008SPIE.7013E..69E,
   author = {{Eisenhauer}, F. and {Perrin}, G. and {Brandner}, W. and {Straubmeier}, C. and 
	{Richichi}, A. and {Gillessen}, S. and {Berger}, J.~P. and {Hippler}, S. and 
	{Eckart}, A. and {Sch{\"o}ller}, M. and {Rabien}, S. and {Cassaing}, F. and 
	{Lenzen}, R. and {Thiel}, M. and {Cl{\'e}net}, Y. and {Ramos}, J.~R. and 
	{Kellner}, S. and {F{\'e}dou}, P. and {Baumeister}, H. and {Hofmann}, R. and 
	{Gendron}, E. and {Boehm}, A. and {Bartko}, H. and {Haubois}, X. and 
	{Klein}, R. and {Dodds-Eden}, K. and {Houairi}, K. and {Hormuth}, F. and 
	{Gr{\"a}ter}, A. and {Jocou}, L. and {Naranjo}, V. and {Genzel}, R. and 
	{Kervella}, P. and {Henning}, T. and {Hamaus}, N. and {Lacour}, S. and 
	{Neumann}, U. and {Haug}, M. and {Malbet}, F. and {Laun}, W. and 
	{Kolmeder}, J. and {Paumard}, T. and {Rohloff}, R.-R. and {Pfuhl}, O. and 
	{Perraut}, K. and {Ziegleder}, J. and {Rouan}, D. and {Rousset}, G.
	},
    title = "{GRAVITY: getting to the event horizon of Sgr A*}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2008,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 7013,
archivePrefix = "arXiv",
   eprint = {0808.0063},
    month = jul,
      eid = {70132A},
      doi = {10.1117/12.788407},
   adsurl = {http://adsabs.harvard.edu/abs/2008SPIE.7013E..69E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2008SPIE.7013E..70L,
   author = {{Lopez}, B. and {Antonelli}, P. and {Wolf}, S. and {Lagarde}, S. and 
	{Jaffe}, W. and {Navarro}, R. and {Graser}, U. and {Petrov}, R. and 
	{Weigelt}, G. and {Bresson}, Y. and {Hofmann}, K.~H. and {Beckman}, U. and 
	{Henning}, T. and {Laun}, W. and {Leinert}, C. and {Kraus}, S. and 
	{Robbe-Dubois}, S. and {Vakili}, F. and {Richichi}, A. and {Abraham}, P. and 
	{Augereau}, J.-C. and {Behrend}, J. and {Berio}, P. and {Berruyer}, N. and 
	{Chesneau}, O. and {Clausse}, J.~M. and {Connot}, C. and {Demyk}, K. and 
	{Danchi}, W.~C. and {Dugu{\'e}}, M. and {Finger}, G. and {Flament}, S. and 
	{Glazenborg}, A. and {Hannenburg}, H. and {Heininger}, M. and 
	{Hugues}, Y. and {Hron}, J. and {Jankov}, S. and {Kerschbaum}, F. and 
	{Kroes}, G. and {Linz}, H. and {Lizon}, J.-L. and {Mathias}, P. and 
	{Mathar}, R. and {Matter}, A. and {Menut}, J.~L. and {Meisenheimer}, K. and 
	{Millour}, F. and {Nardetto}, N. and {Neumann}, U. and {Nussbaum}, E. and 
	{Niedzielski}, A. and {Mosoni}, L. and {Olofsson}, J. and {Rabbia}, Y. and 
	{Ratzka}, T. and {Rigal}, F. and {Roussel}, A. and {Schertl}, D. and 
	{Schmider}, F.-X. and {Stecklum}, B. and {Thiebaut}, E. and 
	{Vannier}, M. and {Valat}, B. and {Wagner}, K. and {Waters}, L.~B.~F.~M.
	},
    title = "{MATISSE: perspective of imaging in the mid-infrared at the VLTI}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2008,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 7013,
    month = jul,
      eid = {70132B},
      doi = {10.1117/12.789412},
   adsurl = {http://adsabs.harvard.edu/abs/2008SPIE.7013E..70L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2004SPIE.5491.1370M,
   author = {{Monnier}, J.~D. and {Berger}, J.-P. and {Millan-Gabet}, R. and 
	{ten Brummelaar}, T.~A.},
    title = "{The Michigan Infrared Combiner (MIRC): IR imaging with the CHARA Array}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2004,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 5491,
   editor = {{Traub}, W.~A.},
    month = oct,
    pages = {1370},
   adsurl = {http://adsabs.harvard.edu/abs/2004SPIE.5491.1370M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1998ApJ...496..550A,
   author = {{Armstrong}, J.~T. and {Mozurkewich}, D. and {Rickard}, L.~J. and 
	{Hutter}, D.~J. and {Benson}, J.~A. and {Bowers}, P.~F. and 
	{Elias}, II, N.~M. and {Hummel}, C.~A. and {Johnston}, K.~J. and 
	{Buscher}, D.~F. and {Clark}, III, J.~H. and {Ha}, L. and {Ling}, L.-C. and 
	{White}, N.~M. and {Simon}, R.~S.},
    title = "{The Navy Prototype Optical Interferometer}",
  journal = {\apj},
 keywords = {INSTRUMENTATION: INTERFEROMETERS, TECHNIQUES: INTERFEROMETRIC},
     year = 1998,
    month = mar,
   volume = 496,
    pages = {550},
      doi = {10.1086/305365},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...496..550A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2008SPIE.7013E..63I,
   author = {{Ireland}, M.~J. and {M{\'e}rand}, A. and {ten Brummelaar}, T.~A. and 
	{Tuthill}, P.~G. and {Schaefer}, G.~H. and {Turner}, N.~H. and 
	{Sturmann}, J. and {Sturmann}, L. and {McAlister}, H.~A.},
    title = "{Sensitive visible interferometry with PAVO}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2008,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 7013,
    month = jul,
      eid = {701324},
      doi = {10.1117/12.788386},
   adsurl = {http://adsabs.harvard.edu/abs/2008SPIE.7013E..63I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...740L...2S,
   author = {{Silva Aguirre}, V. and {Chaplin}, W.~J. and {Ballot}, J. and 
	{Basu}, S. and {Bedding}, T.~R. and {Serenelli}, A.~M. and {Verner}, G.~A. and 
	{Miglio}, A. and {Monteiro}, M.~J.~P.~F.~G. and {Weiss}, A. and 
	{Appourchaux}, T. and {Bonanno}, A. and {Broomhall}, A.~M. and 
	{Bruntt}, H. and {Campante}, T.~L. and {Casagrande}, L. and 
	{Corsaro}, E. and {Elsworth}, Y. and {Garc{\'{\i}}a}, R.~A. and 
	{Gaulme}, P. and {Handberg}, R. and {Hekker}, S. and {Huber}, D. and 
	{Karoff}, C. and {Mathur}, S. and {Mosser}, B. and {Salabert}, D. and 
	{Sch{\"o}nrich}, R. and {Sousa}, S.~G. and {Stello}, D. and 
	{White}, T.~R. and {Christensen-Dalsgaard}, J. and {Gilliland}, R.~L. and 
	{Kawaler}, S.~D. and {Kjeldsen}, H. and {Houdek}, G. and {Metcalfe}, T.~S. and 
	{Molenda-{\.Z}akowicz}, J. and {Thompson}, M.~J. and {Caldwell}, D.~A. and 
	{Christiansen}, J.~L. and {Wohler}, B.},
    title = "{Constructing a One-solar-mass Evolutionary Sequence Using Asteroseismic Data from Kepler}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1108.2031},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, stars: evolution, stars: oscillations},
     year = 2011,
    month = oct,
   volume = 740,
      eid = {L2},
    pages = {L2},
      doi = {10.1088/2041-8205/740/1/L2},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...740L...2S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...537A..30M,
   author = {{Mosser}, B. and {Elsworth}, Y. and {Hekker}, S. and {Huber}, D. and 
	{Kallinger}, T. and {Mathur}, S. and {Belkacem}, K. and {Goupil}, M.~J. and 
	{Samadi}, R. and {Barban}, C. and {Bedding}, T.~R. and {Chaplin}, W.~J. and 
	{Garc{\'{\i}}a}, R.~A. and {Stello}, D. and {De Ridder}, J. and 
	{Middour}, C.~K. and {Morris}, R.~L. and {Quintana}, E.~V.},
    title = "{Characterization of the power excess of solar-like oscillations in red giants with Kepler}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.0980},
 primaryClass = "astro-ph.SR",
 keywords = {stars: oscillations, stars: interiors, stars: evolution, stars: mass-loss, stars: late-type, methods: data analysis},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A30},
    pages = {A30},
      doi = {10.1051/0004-6361/201117352},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A..30M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{1997IAUS..178..441J,
   author = {{J{\o}rgensen}, U.~G.},
    title = "{Cool star models.}",
 keywords = {Cool Stars: Models, Cool Stars: Molecules},
booktitle = {IAU Symposium},
     year = 1997,
   series = {IAU Symposium},
   volume = 178,
   editor = {{van Dishoeck}, E.~F.},
    pages = {441-456},
   adsurl = {http://adsabs.harvard.edu/abs/1997IAUS..178..441J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gaussref,
   author = {{Lowan}, A.~N. and {Davids}, N. and {Levenson}, A.},
    title = "{Table of the zeros of the Legendre polynomials of order 1-16 and the weight coefficients for Gauss' mechanical quadrature}",
  journal = {Bull. Amer. Math. Soc.},
     year = 1942,
   volume = 48,
    pages = {739-743},
   adsurl = {http://www.ams.org/journals/bull/1942-48-10/S0002-9904-1942-07771-8/S0002-9904-1942-07771-8.pdf},
}


@ARTICLE{2010A&A...517A..49H,
   author = {{Hayek}, W. and {Asplund}, M. and {Carlsson}, M. and {Trampedach}, R. and 
	{Collet}, R. and {Gudiksen}, B.~V. and {Hansteen}, V.~H. and 
	{Leenaarts}, J.},
    title = "{Radiative transfer with scattering for domain-decomposed 3D MHD simulations of cool stellar atmospheres. Numerical methods and application to the quiet, non-magnetic, surface of a solar-type star}",
  journal = {\aap},
 keywords = {radiative transfer, stars: atmospheres, Sun: atmosphere},
     year = 2010,
    month = jul,
   volume = 517,
      eid = {A49},
    pages = {A49},
      doi = {10.1051/0004-6361/201014210},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...517A..49H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2001ASPC..223..878S,
   author = {{Stempels}, H.~C. and {Piskunov}, N. and {Barklem}, P.~S.},
    title = "{Recent Developments of the VALD Database (CD-ROM Directory: contribs/stempels)}",
booktitle = {11th Cambridge Workshop on Cool Stars, Stellar Systems and the Sun},
     year = 2001,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 223,
   editor = {{Garcia Lopez}, R.~J. and {Rebolo}, R. and {Zapaterio Osorio}, M.~R.
	},
    pages = {878},
   adsurl = {http://adsabs.harvard.edu/abs/2001ASPC..223..878S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2013A&A...557A..26M,
   author = {{Magic}, Z. and {Collet}, R. and {Asplund}, M. and {Trampedach}, R. and 
	{Hayek}, W. and {Chiavassa}, A. and {Stein}, R.~F. and {Nordlund}, {\AA}.
	},
    title = "{The Stagger-grid: A grid of 3D stellar atmosphere models. I. Methods and general properties}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1302.2621},
 primaryClass = "astro-ph.SR",
 keywords = {convection, hydrodynamics, radiative transfer, stars: abundances, stars: atmospheres, stars: fundamental parameters},
     year = 2013,
    month = sep,
   volume = 557,
      eid = {A26},
    pages = {A26},
      doi = {10.1051/0004-6361/201321274},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...557A..26M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2012A&A...540A...5C,
   author = {{Chiavassa}, A. and {Bigot}, L. and {Kervella}, P. and {Matter}, A. and 
	{Lopez}, B. and {Collet}, R. and {Magic}, Z. and {Asplund}, M.
	},
    title = "{Three-dimensional interferometric, spectrometric, and planetary views of Procyon}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1201.3264},
 primaryClass = "astro-ph.SR",
 keywords = {radiative transfer, hydrodynamics, techniques: interferometric, planetary systems, stars: atmospheres, stars: individual: Procyon},
     year = 2012,
    month = apr,
   volume = 540,
      eid = {A5},
    pages = {A5},
      doi = {10.1051/0004-6361/201118652},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...540A...5C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011JPhCS.328a2012C,
   author = {{Chiavassa}, A. and {Bigot}, L. and {Th{\'e}venin}, F. and {Collet}, R. and 
	{Jasniewicz}, G. and {Magic}, Z. and {Asplund}, M.},
    title = "{3-D hydrodynamical model atmospheres: a tool to correct radial velocities and parallaxes for Gaia}",
  journal = {Journal of Physics Conference Series},
archivePrefix = "arXiv",
   eprint = {1111.5515},
 primaryClass = "astro-ph.SR",
     year = 2011,
    month = dec,
   volume = 328,
   number = 1,
      eid = {012012},
    pages = {012012},
      doi = {10.1088/1742-6596/328/1/012012},
   adsurl = {http://adsabs.harvard.edu/abs/2011JPhCS.328a2012C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...690L.122C,
   author = {{Cami}, J. and {Sloan}, G.~C. and {Markwick-Kemper}, A.~J. and 
	{Zijlstra}, A.~A. and {Bauschlicher}, C.~W. and {Matsuura}, M. and 
	{Decin}, L. and {Hony}, S.},
    title = "{The Detection of Infrared SiS Bands in Spectra of S Stars}",
  journal = {\apjl},
 keywords = {infrared: stars, molecular data, stars: AGB and post-AGB, stars: atmospheres},
     year = 2009,
    month = jan,
   volume = 690,
    pages = {L122-L125},
      doi = {10.1088/0004-637X/690/2/L122},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690L.122C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2010A&A...517A..49H,
   author = {{Hayek}, W. and {Asplund}, M. and {Carlsson}, M. and {Trampedach}, R. and 
	{Collet}, R. and {Gudiksen}, B.~V. and {Hansteen}, V.~H. and 
	{Leenaarts}, J.},
    title = "{Radiative transfer with scattering for domain-decomposed 3D MHD simulations of cool stellar atmospheres. Numerical methods and application to the quiet, non-magnetic, surface of a solar-type star}",
  journal = {\aap},
 keywords = {radiative transfer, stars: atmospheres, Sun: atmosphere},
     year = 2010,
    month = jul,
   volume = 517,
      eid = {A49},
    pages = {A49},
      doi = {10.1051/0004-6361/201014210},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...517A..49H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011arXiv1110.5475C,
   author = {{Collet}, R. and {Magic}, Z. and {Asplund}, M.},
    title = "{The StaggerGrid Project: a Grid of 3D Model Atmospheres for High-Precision Spectroscopy}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1110.5475},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics},
     year = 2011,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2011arXiv1110.5475C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2011arXiv1110.6844F,
   author = {{Freytag}, B. and {Steffen}, M. and {Ludwig}, H.-G. and {Wedemeyer-B{\"o}hm}, S. and 
	{Schaffenberger}, W. and {Steiner}, O.},
    title = "{Simulations of stellar convection with CO5BOLD}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1110.6844},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics},
     year = 2011,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2011arXiv1110.6844F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gelly86,
   author = {{Gelly}, B. and {Grec}, G. and {Fossat}, E.},
    title = "{Evidence for global pressure oscillations in Procyon and Alpha Centauri}",
  journal = {\aap},
 keywords = {HELIOSEISMOLOGY, PRESSURE OSCILLATIONS, STELLAR OSCILLATIONS, STELLAR STRUCTURE, CENTAURUS CONSTELLATION, EARLY STARS, MAIN SEQUENCE STARS, SPECTROPHOTOMETRY},
     year = 1986,
    month = aug,
   volume = 164,
    pages = {383-394},
   adsurl = {http://adsabs.harvard.edu/abs/1986A%26A...164..383G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martic04,
   author = {{Marti{\'c}}, M. and {Lebrun}, J.-C. and {Appourchaux}, T. and 
	{Korzennik}, S.~G.},
    title = "{p-mode frequencies in solar-like stars.  I. Procyon A}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0403035},
 keywords = {stars: oscillations (including pulsations), stars: individual: Procyon A, techniques: radial velocities},
     year = 2004,
    month = apr,
   volume = 418,
    pages = {295-303},
      doi = {10.1051/0004-6361:20034574},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...418..295M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{gelly88,
   author = {{Gelly}, B. and {Grec}, G. and {Fossat}, E.},
    title = "{Evidence for Global Pressure Oscillations in Procyon and Alpha-Centauri}",
booktitle = {Advances in Helio- and Asteroseismology},
     year = 1988,
   series = {IAU Symposium},
   volume = 123,
   editor = "{J.~Christensen-Dalsgaard \& S.~Frandsen}",
    pages = {249},
   adsurl = {http://adsabs.harvard.edu/abs/1988IAUS..123..249G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011arXiv1110.5475C,
   author = {{Collet}, R. and {Magic}, Z. and {Asplund}, M.},
    title = "{The StaggerGrid Project: a Grid of 3D Model Atmospheres for High-Precision Spectroscopy}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1110.5475},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics},
     year = 2011,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2011arXiv1110.5475C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006A&A...446..635B,
   author = {{Bigot}, L. and {Kervella}, P. and {Th{\'e}venin}, F. and {S{\'e}gransan}, D.
	},
    title = "{The limb darkening of {$\alpha$} Centauri B. Matching 3D hydrodynamical models with interferometric measurements}",
  journal = {\aap},
 keywords = {instrumentation: interferometers, stars: atmospheres},
     year = 2006,
    month = feb,
   volume = 446,
    pages = {635-641},
      doi = {10.1051/0004-6361:20053187},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...446..635B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2011A&A...534L...3B,
   author = {{Bigot}, L. and {Mourard}, D. and {Berio}, P. and {Th{\'e}venin}, F. and 
	{Ligi}, R. and {Tallon-Bosc}, I. and {Chesneau}, O. and {Delaa}, O. and 
	{Nardetto}, N. and {Perraut}, K. and {Stee}, P. and {Boyajian}, T. and 
	{Morel}, P. and {Pichon}, B. and {Kervella}, P. and {Schmider}, F.~X. and 
	{McAlister}, H. and {Ten Brummelaar}, T. and {Ridgway}, S.~T. and 
	{Sturmann}, J. and {Sturmann}, L. and {Turner}, N. and {Farrington}, C. and 
	{Goldfinger}, P.~J.},
    title = "{The diameter of the CoRoT target HD 49933. Combining the 3D limb darkening, asteroseismology, and interferometry}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.0985},
 primaryClass = "astro-ph.SR",
 keywords = {stars: oscillations, hydrodynamics, stars: fundamental parameters, techniques: interferometric, asteroseismology, stars: individual: HD 49933},
     year = 2011,
    month = oct,
   volume = 534,
      eid = {L3},
    pages = {L3},
      doi = {10.1051/0004-6361/201117349},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...534L...3B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2005ApJ...618..926S,
   author = {{Short}, C.~I. and {Hauschildt}, P.~H.},
    title = "{A Non-LTE Line-Blanketed Model of a Solar-Type Star}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0409693},
 keywords = {Line: Formation, Radiative Transfer, Stars: Atmospheres, Stars: Late-Type, Sun: Atmosphere},
     year = 2005,
    month = jan,
   volume = 618,
    pages = {926-938},
      doi = {10.1086/426128},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...618..926S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2001ApJ...556..357A,
   author = {{Allard}, F. and {Hauschildt}, P.~H. and {Alexander}, D.~R. and 
	{Tamanai}, A. and {Schweitzer}, A.},
    title = "{The Limiting Effects of Dust in Brown Dwarf Model Atmospheres}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0104256},
 keywords = {Stars: Atmospheres, Stars: Fundamental Parameters, Stars: Low-Mass, Brown Dwarfs},
     year = 2001,
    month = jul,
   volume = 556,
    pages = {357-372},
      doi = {10.1086/321547},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...556..357A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{provencal02,
   author = {{Provencal}, J.~L. and {Shipman}, H.~L. and {Koester}, D. and 
	{Wesemael}, F. and {Bergeron}, P.},
    title = "{Procyon B: Outside the Iron Box}",
  journal = {\apj},
 keywords = {Stars: Individual: Name: Procyon B, Stars: White Dwarfs},
     year = 2002,
    month = mar,
   volume = 568,
    pages = {324-334},
      doi = {10.1086/338769},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...568..324P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{griffin71,
   author = {{Griffin}, R.},
    title = "{Curve-of-growth analysis of the spectrum of Procyon.}",
  journal = {\mnras},
     year = 1971,
   volume = 155,
    pages = {139-152},
   adsurl = {http://adsabs.harvard.edu/abs/1971MNRAS.155..139G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gray67,
   author = {{Gray}, D.~F.},
    title = "{Photometric Determination of Stellar Radii}",
  journal = {\apj},
     year = 1967,
    month = aug,
   volume = 149,
    pages = {317},
      doi = {10.1086/149256},
   adsurl = {http://adsabs.harvard.edu/abs/1967ApJ...149..317G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{strand51,
   author = {{Strand}, K.~A.},
    title = "{The Orbit and Parallax of Procyon.}",
  journal = {\apj},
     year = 1951,
    month = jan,
   volume = 113,
    pages = {1},
      doi = {10.1086/145373},
   adsurl = {http://adsabs.harvard.edu/abs/1951ApJ...113....1S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{code76,
   author = {{Code}, A.~D. and {Bless}, R.~C. and {Davis}, J. and {Brown}, R.~H.
	},
    title = "{Empirical effective temperatures and bolometric corrections for early-type stars}",
  journal = {\apj},
 keywords = {BOLOMETERS, EARLY STARS, RADIANT FLUX DENSITY, SPECTRAL ENERGY DISTRIBUTION, STELLAR SPECTROPHOTOMETRY, STELLAR TEMPERATURE, ASTRONOMICAL CATALOGS, INFRARED SPECTROSCOPY, OAO 2, STELLAR ATMOSPHERES, STELLAR LUMINOSITY, STELLAR STRUCTURE, ULTRAVIOLET SPECTROSCOPY},
     year = 1976,
    month = jan,
   volume = 203,
    pages = {417-434},
      doi = {10.1086/154093},
   adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...203..417C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gatewood06,
   author = {{Gatewood}, G. and {Han}, I.},
    title = "{An Astrometric Study of Procyon}",
  journal = {\aj},
 keywords = {Stars: Binaries: Spectroscopic, Stars: Binaries: Visual, Stars: Individual: Name: Procyon},
     year = 2006,
    month = feb,
   volume = 131,
    pages = {1015-1021},
      doi = {10.1086/498894},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....131.1015G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{schaeberle1896,
   author = {{Schaeberle}, J.~M.},
    title = "{Discovery of the companion to Procyon}",
  journal = {\aj},
     year = 1896,
    month = dec,
   volume = 17,
    pages = {37-37},
      doi = {10.1086/102580},
   adsurl = {http://adsabs.harvard.edu/abs/1896AJ.....17...37S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1997ApJ...480..777P,
   author = {{Provencal}, J.~L. and {Shipman}, H.~L. and {Wesemael}, F. and 
	{Bergeron}, P. and {Bond}, H.~E. and {Liebert}, J. and {Sion}, E.~M.
	},
    title = "{Wide Field Planetary Camera 2 Photometry of the Bright, Mysterious White Dwarf Procyon B}",
  journal = {\apj},
 keywords = {STARS: INTERIORS, STARS: INDIVIDUAL NAME: PROCYON B, STARS: WHITE DWARFS, ULTRAVIOLET: STARS},
     year = 1997,
    month = may,
   volume = 480,
    pages = {777},
      doi = {10.1086/304003},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...480..777P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000A&A...363.1081C,
   author = {{Claret}, A.},
    title = "{A new non-linear limb-darkening law for LTE stellar atmosphere models. Calculations for -5.0 {\lt}= log[M/H] {\lt}= +1, 2000 K {\lt}= T$_{eff}$ {\lt}= 50000 K at several surface gravities}",
  journal = {\aap},
 keywords = {STARS: ATMOSPHERES, STARS: BINARIES: ECLIPSING},
     year = 2000,
    month = nov,
   volume = 363,
    pages = {1081-1190},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...363.1081C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2001ApJ...556..885B,
   author = {{Barman}, T.~S. and {Hauschildt}, P.~H. and {Allard}, F.},
    title = "{Irradiated Planets}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0104262},
 keywords = {Stars: Planetary Systems, Radiative Transfer, Stars: Atmospheres},
     year = 2001,
    month = aug,
   volume = 556,
    pages = {885-895},
      doi = {10.1086/321610},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...556..885B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2010SPIE.7734E..99B,
   author = {{Berger}, J.-P. and {Zins}, G. and {Lazareff}, B. and {Lebouquin}, J.-B. and 
	{Jocou}, L. and {Kern}, P. and {Millan-Gabet}, R. and {Traub}, W. and 
	{Haguenauer}, P. and {Absil}, O. and {Augereau}, J.-C. and {Benisty}, M. and 
	{Blind}, N. and {Bonfils}, X. and {Delboulbe}, A. and {Feautrier}, P. and 
	{Germain}, M. and {Gillier}, D. and {Gitton}, P. and {Kiekebusch}, M. and 
	{Knudstrup}, J. and {Lizon}, J.-L. and {Magnard}, Y. and {Malbet}, F. and 
	{Maurel}, D. and {Menard}, F. and {Micallef}, M. and {Michaud}, L. and 
	{Morel}, S. and {Moulin}, T. and {Popovic}, D. and {Perraut}, K. and 
	{Rabou}, P. and {Rochat}, S. and {Roussel}, F. and {Roux}, A. and 
	{Stadler}, E. and {Tatulli}, E.},
    title = "{PIONIER: a visitor instrument for VLTI}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2010,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 7734,
archivePrefix = "arXiv",
   eprint = {1008.5352},
 primaryClass = "astro-ph.IM",
    month = jul,
      eid = {773435},
      doi = {10.1117/12.858647},
   adsurl = {http://adsabs.harvard.edu/abs/2010SPIE.7734E..99B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2008SPIE.7013E..11H,
   author = {{Haguenauer}, P. and {Abuter}, R. and {Alonso}, J. and {Argomedo}, J. and 
	{Bauvir}, B. and {Blanchard}, G. and {Bonnet}, H. and {Brillant}, S. and 
	{Cantzler}, M. and {Derie}, F. and {Delplancke}, F. and {Di Lieto}, N. and 
	{Dupuy}, C. and {Durand}, Y. and {Gitton}, P. and {Gilli}, B. and 
	{Glindemann}, A. and {Guniat}, S. and {Guisard}, S. and {Haddad}, N. and 
	{Hudepohl}, G. and {Hummel}, C. and {Jesuran}, N. and {Kaufer}, A. and 
	{Koehler}, B. and {Le Bouquin}, J.-B. and {L{\'e}v''que}, S. and 
	{Lidman}, C. and {Mardones}, P. and {M{\'e}nardi}, S. and {Morel}, S. and 
	{Percheron}, I. and {Petr-Gotzens}, M. and {Phan Duc}, T. and 
	{Puech}, F. and {Ramirez}, A. and {Rantakyr{\"o}}, F. and {Richichi}, A. and 
	{Rivinius}, T. and {Sahlmann}, J. and {Sandrock}, S. and {Sch{\"o}ller}, M. and 
	{Schuhler}, N. and {Somboli}, F. and {Stefl}, S. and {Tapia}, M. and 
	{Van Belle}, G. and {Wallander}, A. and {Wehner}, S. and {Wittkowski}, M.
	},
    title = "{The Very Large Telescope Interferometer: an update}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2008,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 7013,
    month = jul,
      eid = {70130C},
      doi = {10.1117/12.788209},
   adsurl = {http://adsabs.harvard.edu/abs/2008SPIE.7013E..11H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2011A&A...535A..68A,
   author = {{Absil}, O. and {Le Bouquin}, J.-B. and {Berger}, J.-P. and 
	{Lagrange}, A.-M. and {Chauvin}, G. and {Lazareff}, B. and {Zins}, G. and 
	{Haguenauer}, P. and {Jocou}, L. and {Kern}, P. and {Millan-Gabet}, R. and 
	{Rochat}, S. and {Traub}, W.},
    title = "{Searching for faint companions with VLTI/PIONIER. I. Method and first results}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.1178},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: interferometric, binaries: close, stars: low mass, brown dwarfs, planetary systems},
     year = 2011,
    month = nov,
   volume = 535,
      eid = {A68},
    pages = {A68},
      doi = {10.1051/0004-6361/201117719},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...535A..68A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011PASP..123..964Z,
   author = {{Zhao}, M. and {Monnier}, J.~D. and {Che}, X. and {Pedretti}, E. and 
	{Thureau}, N. and {Schaefer}, G. and {Ten Brummelaar}, T. and 
	{M{\'e}rand}, A. and {Ridgway}, S.~T. and {McAlister}, H. and 
	{Turner}, N. and {Sturmann}, J. and {Sturmann}, L. and {Goldfinger}, P.~J. and 
	{Farrington}, C.},
    title = "{Toward Direct Detection of Hot Jupiters with Precision Closure Phase: Calibration Studies and First Results from the CHARA Array}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1109.5183},
 primaryClass = "astro-ph.EP",
     year = 2011,
    month = aug,
   volume = 123,
    pages = {964-975},
      doi = {10.1086/661762},
   adsurl = {http://adsabs.harvard.edu/abs/2011PASP..123..964Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...515A..69M,
   author = {{Matter}, A. and {Vannier}, M. and {Morel}, S. and {Lopez}, B. and 
	{Jaffe}, W. and {Lagarde}, S. and {Petrov}, R.~G. and {Leinert}, C.
	},
    title = "{First step to detect an extrasolar planet using simultaneous observations with the VLTI instruments AMBER and MIDI}",
  journal = {\aap},
 keywords = {instrumentation: interferometers, techniques: interferometric, planetary systems, infrared: general, atmospheric effects},
     year = 2010,
    month = jun,
   volume = 515,
      eid = {A69},
    pages = {A69},
      doi = {10.1051/0004-6361/200913142},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...515A..69M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2004SPIE.5491..551J,
   author = {{Joergens}, V. and {Quirrenbach}, A.},
    title = "{Modeling of closure phase measurements with AMBER/VLTI: toward characterization of exoplanetary atmospheres}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2004,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 5491,
   eprint = {arXiv:astro-ph/0409726},
   editor = "{W.~A.~Traub}",
    month = oct,
    pages = {551},
   adsurl = {http://adsabs.harvard.edu/abs/2004SPIE.5491..551J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ApJ...678.1436B,
   author = {{Burrows}, A. and {Budaj}, J. and {Hubeny}, I.},
    title = "{Theoretical Spectra and Light Curves of Close-in Extrasolar Giant Planets and Comparison with Data}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0709.4080},
 keywords = {Stars: Planetary Systems, Planets and Satellites: General, Stars: Individual: Henry Draper Number: HD 209458, stars: individual (HD 189733), Stars: Individual: Alphanumeric: TrES-1, stars: individual (HD 149026), Stars: Individual: Constellation Name: {\upsi} Andromedae, Stars: Individual: Henry Draper Number: HD 179949},
     year = 2008,
    month = may,
   volume = 678,
    pages = {1436-1457},
      doi = {10.1086/533518},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...678.1436B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1995Natur.378..355M,
   author = {{Mayor}, M. and {Queloz}, D.},
    title = "{A Jupiter-mass companion to a solar-type star}",
  journal = {\nat},
     year = 1995,
    month = nov,
   volume = 378,
    pages = {355-359},
      doi = {10.1038/378355a0},
   adsurl = {http://adsabs.harvard.edu/abs/1995Natur.378..355M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2008SPIE.7013E..45Z,
   author = {{Zhao}, M. and {Monnier}, J.~D. and {ten Brummelaar}, T. and 
	{Pedretti}, E. and {Thureau}, N.~D.},
    title = "{Exoplanet studies with CHARA-MIRC}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2008,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 7013,
    month = jul,
      doi = {10.1117/12.789698},
   adsurl = {http://adsabs.harvard.edu/abs/2008SPIE.7013E..45Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003RPPh...66..789M,
   author = {{Monnier}, J.~D.},
    title = "{Optical interferometry in astronomy}",
  journal = {Reports on Progress in Physics},
   eprint = {arXiv:astro-ph/0307036},
     year = 2003,
    month = may,
   volume = 66,
    pages = {789-857},
      doi = {10.1088/0034-4885/66/5/203},
   adsurl = {http://adsabs.harvard.edu/abs/2003RPPh...66..789M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...628..453T,
   author = {{ten Brummelaar}, T.~A. and {McAlister}, H.~A. and {Ridgway}, S.~T. and 
	{Bagnuolo}, Jr., W.~G. and {Turner}, N.~H. and {Sturmann}, L. and 
	{Sturmann}, J. and {Berger}, D.~H. and {Ogden}, C.~E. and {Cadman}, R. and 
	{Hartkopf}, W.~I. and {Hopper}, C.~H. and {Shure}, M.~A.},
    title = "{First Results from the CHARA Array. II. A Description of the Instrument}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0504082},
 keywords = {Atmospheric Effects, Instrumentation: High Angular Resolution, Instrumentation: Interferometers, Techniques: High Anular Resolution, Techniques: Interferometric, Telescopes},
     year = 2005,
    month = jul,
   volume = 628,
    pages = {453-465},
      doi = {10.1086/430729},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...628..453T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2003yCat.2246....0C,
   author = {{Cutri}, R.~M. and {Skrutskie}, M.~F. and {van Dyk}, S. and 
	{Beichman}, C.~A. and {Carpenter}, J.~M. and {Chester}, T. and 
	{Cambresy}, L. and {Evans}, T. and {Fowler}, J. and {Gizis}, J. and 
	{Howard}, E. and {Huchra}, J. and {Jarrett}, T. and {Kopan}, E.~L. and 
	{Kirkpatrick}, J.~D. and {Light}, R.~M. and {Marsh}, K.~A. and 
	{McCallon}, H. and {Schneider}, S. and {Stiening}, R. and {Sykes}, M. and 
	{Weinberg}, M. and {Wheaton}, W.~A. and {Wheelock}, S. and {Zacarias}, N.
	},
    title = "{2MASS All-Sky Catalog of Point Sources (Cutri+ 2003)}",
  journal = {VizieR Online Data Catalog},
 keywords = {out.sam          1000x382  2MASS Point Source Catalogue, sample output (on a total of 470,992,970 sources)},
     year = 2003,
    month = mar,
   volume = 2246,
    pages = {0},
   adsurl = {http://adsabs.harvard.edu/abs/2003yCat.2246....0C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...508.1073M,
   author = {{Mourard}, D. and {Clausse}, J.~M. and {Marcotto}, A. and {Perraut}, K. and 
	{Tallon-Bosc}, I. and {B{\'e}rio}, P. and {Blazit}, A. and {Bonneau}, D. and 
	{Bosio}, S. and {Bresson}, Y. and {Chesneau}, O. and {Delaa}, O. and 
	{H{\'e}nault}, F. and {Hughes}, Y. and {Lagarde}, S. and {Merlin}, G. and 
	{Roussel}, A. and {Spang}, A. and {Stee}, P. and {Tallon}, M. and 
	{Antonelli}, P. and {Foy}, R. and {Kervella}, P. and {Petrov}, R. and 
	{Thiebaut}, E. and {Vakili}, F. and {McAlister}, H. and {ten Brummelaar}, T. and 
	{Sturmann}, J. and {Sturmann}, L. and {Turner}, N. and {Farrington}, C. and 
	{Goldfinger}, P.~J.},
    title = "{VEGA: Visible spEctroGraph and polArimeter for the CHARA array: principle and performance}",
  journal = {\aap},
 keywords = {instrumentation: high angular resolution, instrumentation: interferometers},
     year = 2009,
    month = dec,
   volume = 508,
    pages = {1073-1083},
      doi = {10.1051/0004-6361/200913016},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...508.1073M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2001ARA&A..39..353Q,
   author = {{Quirrenbach}, A.},
    title = "{Optical Interferometry}",
  journal = {\araa},
 keywords = {ASTRONOMICAL INSTRUMENTATION, ASTROMETRY, STELLAR PARAMETERS, BINARY STARS, CIRCUMSTELLAR MATTER},
     year = 2001,
   volume = 39,
    pages = {353-401},
      doi = {10.1146/annurev.astro.39.1.353},
   adsurl = {http://adsabs.harvard.edu/abs/2001ARA%26A..39..353Q},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2003A&A...408..681K,
   author = {{Kervella}, P. and {Th{\'e}venin}, F. and {Morel}, P. and {Bord{\'e}}, P. and 
	{Di Folco}, E.},
    title = "{The interferometric diameter and internal structure of Sirius A}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0306604},
 keywords = {stars: individual: Sirius, stars: fundamental parameters, stars: evolution, techniques: interferometric},
     year = 2003,
    month = sep,
   volume = 408,
    pages = {681-688},
      doi = {10.1051/0004-6361:20030994},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...408..681K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003A&A...404.1087K,
   author = {{Kervella}, P. and {Th{\'e}venin}, F. and {S{\'e}gransan}, D. and 
	{Berthomieu}, G. and {Lopez}, B. and {Morel}, P. and {Provost}, J.
	},
    title = "{The diameters of alpha  Centauri A and B. A comparison of the asteroseismic and VINCI/VLTI views}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0303634},
 keywords = {techniques: interferometric, stars: binaries: visual, stars: evolution, stars: oscillations, stars: fundamental parameters, stars: individual: alpha Cen},
     year = 2003,
    month = jun,
   volume = 404,
    pages = {1087-1097},
      doi = {10.1051/0004-6361:20030570},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...404.1087K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004A&A...413..711W,
   author = {{Wittkowski}, M. and {Aufdenberg}, J.~P. and {Kervella}, P.},
    title = "{Tests of stellar model atmospheres by optical interferometry. VLTI/VINCI limb-darkening measurements of the M4 giant {$\psi$} Phe}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0310128},
 keywords = {techniques: interferometric, stars: atmospheres, stars: fundamental parameters, stars: late-type},
     year = 2004,
    month = jan,
   volume = 413,
    pages = {711-723},
      doi = {10.1051/0004-6361:20034149},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...413..711W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1990A&AS...83..357B,
   author = {{Bessel}, M.~S.},
    title = "{BVRI photometry of the Gliese Catalogue stars}",
  journal = {\aaps},
 keywords = {ASTRONOMICAL CATALOGS, ASTRONOMICAL PHOTOMETRY, ASTRONOMICAL OBSERVATORIES, RED DWARF STARS, SOUTHERN SKY, STELLAR COLOR, STELLAR MAGNITUDE},
     year = 1990,
    month = may,
   volume = 83,
    pages = {357-378},
   adsurl = {http://adsabs.harvard.edu/abs/1990A%26AS...83..357B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991AJ....101.2207M,
   author = {{Mozurkewich}, D. and {Johnston}, K.~J. and {Simon}, R.~S. and 
	{Bowers}, P.~F. and {Gaume}, R. and {Hutter}, D.~J. and {Colavita}, M.~M. and 
	{Shao}, M. and {Pan}, X.~P.},
    title = "{Angular diameter measurements of stars}",
  journal = {\aj},
 keywords = {ASTROMETRY, DIAMETERS, STELLAR STRUCTURE, INTERFEROMETRY, LIMB DARKENING, STELLAR ATMOSPHERES},
     year = 1991,
    month = jun,
   volume = 101,
    pages = {2207-2219},
      doi = {10.1086/115843},
   adsurl = {http://adsabs.harvard.edu/abs/1991AJ....101.2207M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1988A&A...193..357S,
   author = {{Shao}, M. and {Colavita}, M.~M. and {Hines}, B.~E. and {Staelin}, D.~H. and 
	{Hutter}, D.~J. and {Johnston}, K.~J. and {Mozurkewich}, D. and 
	{Simon}, R.~S. and {Hershey}, J.~L. and {Hughes}, J.~A. and 
	{Kaplan}, G.~H.},
    title = "{The Mark III stellar interferometer}",
  journal = {\aap},
 keywords = {ASTROMETRY, INTERFEROMETERS, DELAY LINES, FEEDBACK CONTROL, LASER INTERFEROMETRY, PHASE COHERENCE, POINTING CONTROL SYSTEMS, STAR TRACKERS, STELLAR MOTIONS},
     year = 1988,
    month = mar,
   volume = 193,
    pages = {357-371},
   adsurl = {http://adsabs.harvard.edu/abs/1988A%26A...193..357S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{girard00,
   author = {{Girard}, T.~M. and {Wu}, H. and {Lee}, J.~T. and {Dyson}, S.~E. and 
    {van Altena}, W.~F. and {Horch}, E.~P. and {Gilliland}, R.~L. and 
    {Schaefer}, K.~G. and {Bond}, H.~E. and {Ftaclas}, C. and {Brown}, R.~H. and 
    {Toomey}, D.~W. and {Shipman}, H.~L. and {Provencal}, J.~L. and 
    {Pourbaix}, D.},
    title = "{A Redetermination of the Mass of Procyon}",
  journal = {\aj},
 keywords = {ASTROMETRY, STARS: INDIVIDUAL (PROCYON)},
     year = 2000,
    month = may,
   volume = 119,
    pages = {2428-2436},
      doi = {10.1086/301353},
   adsurl = {http://adsabs.harvard.edu/abs/2000AJ....119.2428G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{dimauro01,
   author = {{di Mauro}, M.~P. and {Christensen-Dalsgaard}, J.},
    title = "{Structure of Procyon A by a Seismological Approach}",
booktitle = {Recent Insights into the Physics of the Sun and Heliosphere: Highlights from SOHO and Other Space Missions},
     year = 2001,
   series = {IAU Symposium},
   volume = 203,
   editor = "{P.~Brekke, B.~Fleck, \& J.~B.~Gurman}",
    pages = {94},
   adsurl = {http://adsabs.harvard.edu/abs/2001IAUS..203...94D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{guenther93,
   author = {{Guenther}, D.~B. and {Demarque}, P.},
    title = "{Evolution and seismology of Procyon}",
  journal = {\apj},
 keywords = {F STARS, STELLAR EVOLUTION, STELLAR MODELS, STELLAR OSCILLATIONS, STELLAR PHYSICS, OPACITY, STELLAR COMPOSITION, STELLAR CONVECTION, STELLAR ENVELOPES, STELLAR INTERIORS, STELLAR MASS},
     year = 1993,
    month = mar,
   volume = 405,
    pages = {298-306},
      doi = {10.1086/172362},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...405..298G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{bonanno07,
   author = {{Bonanno}, A. and {K{\"u}ker}, M. and {Patern{\`o}}, L.},
    title = "{Seismic inference of differential rotation in Procyon A}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0610353},
 keywords = {stars: interiors, stars: evolution, stars: rotation, stars: oscillations, stars: individual: Procyon A},
     year = 2007,
    month = feb,
   volume = 462,
    pages = {1031-1037},
      doi = {10.1051/0004-6361:20065892},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...462.1031B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{martic99,
   author = {{Marti{\'c}}, M. and {Schmitt}, J. and {Lebrun}, J.-C. and {Barban}, C. and 
    {Connes}, P. and {Bouchy}, F. and {Michel}, E. and {Baglin}, A. and 
    {Appourchaux}, T. and {Bertaux}, J.-L.},
    title = "{Evidence for global pressure oscillations on Procyon}",
  journal = {\aap},
 keywords = {STARS: OSCILLATIONS, STARS: INDIVIDUAL: PROCYON, TECHNIQUES: SPECTROSCOPIC},
     year = 1999,
    month = nov,
   volume = 351,
    pages = {993-1002},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...351..993M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{eggenberger04,
   author = {{Eggenberger}, P. and {Carrier}, F. and {Bouchy}, F. and {Blecha}, A.
	},
    title = "{Solar-like oscillations in Procyon A}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0501271},
 keywords = {stars: oscillations, stars: individual: {$\alpha$} Canis Minoris, techniques: radial velocities},
     year = 2004,
    month = jul,
   volume = 422,
    pages = {247-252},
      doi = {10.1051/0004-6361:20040148},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...422..247E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{eggenberger05,
   author = {{Eggenberger}, P. and {Carrier}, F. and {Bouchy}, F.},
    title = "{Models of Procyon A including seismic constraints}",
  journal = {\na},
   eprint = {arXiv:astro-ph/0501270},
 keywords = {97.10.Cv, 97.10.Sj},
     year = 2005,
    month = jan,
   volume = 10,
    pages = {195-208},
      doi = {10.1016/j.newast.2004.10.002},
   adsurl = {http://adsabs.harvard.edu/abs/2005NewA...10..195E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004A&A...413..251K,
   author = {{Kervella}, P. and {Th{\'e}venin}, F. and {Morel}, P. and {Berthomieu}, G. and 
	{Bord{\'e}}, P. and {Provost}, J.},
    title = "{The diameter and evolutionary state of Procyon A. Multi-technique modeling using asteroseismic and interferometric constraints}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0309148},
 keywords = {stars: individual: {$\alpha$} CMi, stars: fundamental parameters, stars: evolution, techniques: interferometric},
     year = 2004,
    month = jan,
   volume = 413,
    pages = {251-256},
      doi = {10.1051/0004-6361:20031527},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...413..251K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hartmann75,
   author = {{Hartmann}, L. and {Garrison}, Jr., L.~M. and {Katz}, A.},
    title = "{On the evolution and composition of Sirius and Procyon}",
  journal = {\apj},
 keywords = {ABUNDANCE, ASTRONOMICAL MODELS, STELLAR EVOLUTION, STELLAR MASS, CHEMICAL COMPOSITION, HERTZSPRUNG-RUSSELL DIAGRAM, MAIN SEQUENCE STARS, METALS, STELLAR STRUCTURE},
     year = 1975,
    month = jul,
   volume = 199,
    pages = {127-130},
      doi = {10.1086/153671},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...199..127H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009LRSP....6....2N,
   author = {{Nordlund}, {\AA}. and {Stein}, R.~F. and {Asplund}, M.},
    title = "{Solar Surface Convection}",
  journal = {Living Reviews in Solar Physics},
 keywords = {solar physics, convection, granulation, mesogranulation, supergranulation},
     year = 2009,
    month = apr,
   volume = 6,
    pages = {2},
   adsurl = {http://adsabs.harvard.edu/abs/2009LRSP....6....2N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{nordlund90,
   author = {{Nordlund}, A. and {Dravins}, D.},
    title = "{Stellar granulation. III - Hydrodynamic model atmospheres. IV - Line formation in inhomogeneous stellar photospheres. V - Synthetic spectral lines in disk-integrated starlight}",
  journal = {\aap},
 keywords = {ASTRONOMICAL MODELS, HYDRODYNAMICS, LATE STARS, SOLAR GRANULATION, STELLAR ATMOSPHERES, F STARS, G STARS, RADIATIVE TRANSFER, STELLAR MAGNETIC FIELDS, STELLAR TEMPERATURE, SUBGIANT STARS},
     year = 1990,
    month = feb,
   volume = 228,
    pages = {155-217},
   adsurl = {http://adsabs.harvard.edu/abs/1990A%26A...228..155N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bessel1844,
   author = {{Bessel}, F.~W.},
    title = "{On the variations of the proper motions of Procyon and Sirius}",
  journal = {\mnras},
     year = 1844,
    month = dec,
   volume = 6,
    pages = {136-141},
   adsurl = {http://adsabs.harvard.edu/abs/1844MNRAS...6R.136B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bedding10,
   author = {{Bedding}, T.~R. and {Kjeldsen}, H. and {Campante}, T.~L. and 
    {Appourchaux}, T. and {Bonanno}, A. and {Chaplin}, W.~J. and 
    {Garcia}, R.~A. and {Marti{\'c}}, M. and {Mosser}, B. and {Butler}, R.~P. and 
    {Bruntt}, H. and {Kiss}, L.~L. and {O'Toole}, S.~J. and {Kambe}, E. and 
    {Ando}, H. and {Izumiura}, H. and {Sato}, B. and {Hartmann}, M. and 
    {Hatzes}, A. and {Barban}, C. and {Berthomieu}, G. and {Michel}, E. and 
    {Provost}, J. and {Turck-Chi{\`e}ze}, S. and {Lebrun}, J.-C. and 
    {Schmitt}, J. and {Bertaux}, J.-L. and {Benatti}, S. and {Claudi}, R.~U. and 
    {Cosentino}, R. and {Leccia}, S. and {Frandsen}, S. and {Brogaard}, K. and 
    {Glowienka}, L. and {Grundahl}, F. and {Stempels}, E. and {Arentoft}, T. and 
    {Bazot}, M. and {Christensen-Dalsgaard}, J. and {Dall}, T.~H. and 
    {Karoff}, C. and {Lundgreen-Nielsen}, J. and {Carrier}, F. and 
    {Eggenberger}, P. and {Sosnowska}, D. and {Wittenmyer}, R.~A. and 
    {Endl}, M. and {Metcalfe}, T.~S. and {Hekker}, S. and {Reffert}, S.
    },
    title = "{A Multi-Site Campaign to Measure Solar-Like Oscillations in Procyon. II. Mode Frequencies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1003.0052},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: Procyon A, stars: oscillations},
     year = 2010,
    month = apr,
   volume = 713,
    pages = {935-949},
      doi = {10.1088/0004-637X/713/2/935},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...713..935B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{guenther08,
   author = {{Guenther}, D.~B. and {Kallinger}, T. and {Gruberbauer}, M. and 
    {Huber}, D. and {Weiss}, W.~W. and {Kuschnig}, R. and {Demarque}, P. and 
    {Robinson}, F. and {Matthews}, J.~M. and {Moffat}, A.~F.~J. and 
    {Rucinski}, S.~M. and {Sasselov}, D. and {Walker}, G.~A.~H.},
    title = "{The Nature of p-modes and Granulation in Procyon: New MOST Photometry and New Yale Convection Models}",
  journal = {\apj},
 keywords = {Convection, Stars: Individual: Name: Procyon, Stars: Interiors, Stars: Oscillations},
     year = 2008,
    month = nov,
   volume = 687,
    pages = {1448-1459},
      doi = {10.1086/592060},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...687.1448G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{provost06,
   author = {{Provost}, J. and {Berthomieu}, G. and {Marti{\'c}}, M. and 
    {Morel}, P.},
    title = "{Asteroseismology and evolutionary status of Procyon A}",
  journal = {\aap},
 keywords = {stars: oscillations, stars: evolution, stars: individual: Procyon A},
     year = 2006,
    month = dec,
   volume = 460,
    pages = {759-767},
      doi = {10.1051/0004-6361:20065251},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...460..759P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2002ApJ...567..544A,
   author = {{Allende Prieto}, C. and {Asplund}, M. and {Garc{\'{\i}}a L{\'o}pez}, R.~J. and 
	{Lambert}, D.~L.},
    title = "{Signatures of Convection in the Spectrum of Procyon: Fundamental Parameters and Iron Abundance}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0111055},
 keywords = {Convection, Line: Formation, Line: Profiles, Stars: Abundances, Stars: Atmospheres, stars: individual (Procyon A)},
     year = 2002,
    month = mar,
   volume = 567,
    pages = {544-565},
      doi = {10.1086/338248},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...567..544A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{nelson80,
   author = {{Nelson}, G.~D.},
    title = "{Granulation in a main-sequence F-type star}",
  journal = {\apj},
 keywords = {CONVECTION CURRENTS, F STARS, MAIN SEQUENCE STARS, PHOTOSPHERE, STELLAR ATMOSPHERES, STELLAR MODELS, STELLAR STRUCTURE, SPECTRAL ENERGY DISTRIBUTION, STELLAR MAGNETIC FIELDS, STELLAR TEMPERATURE, SURFACE LAYERS, TEMPERATURE GRADIENTS},
     year = 1980,
    month = jun,
   volume = 238,
    pages = {659-666},
      doi = {10.1086/158022},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...238..659N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{atroshchenko89,
   author = {{Atroshchenko}, I.~N. and {Gadun}, A.~S. and {Kostik}, R.~I.
	},
    title = "{Three-Dimensional Simulation of Convective Motions in the Procyon Envelope}",
booktitle = {NATO ASIC Proc. 263: Solar and Stellar Granulation},
     year = 1989,
   editor = "{R.~J.~Rutten \& G.~Severino}",
    pages = {521},
   adsurl = {http://adsabs.harvard.edu/abs/1989ssg..conf..521A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2010A&A...512A..54C,
   author = {{Casagrande}, L. and {Ram{\'{\i}}rez}, I. and {Mel{\'e}ndez}, J. and 
	{Bessell}, M. and {Asplund}, M.},
    title = "{An absolutely calibrated T$_{eff}$ scale from the infrared flux method. Dwarfs and subgiants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1001.3142},
 primaryClass = "astro-ph.SR",
 keywords = {stars: fundamental parameters, stars: abundances, stars: atmospheres, infrared: stars, techniques: photometric},
     year = 2010,
    month = mar,
   volume = 512,
      eid = {A54},
    pages = {A54},
      doi = {10.1051/0004-6361/200913204},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...512A..54C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2004A&A...425.1161K,
   author = {{Kervella}, P. and {S{\'e}gransan}, D. and {Coud{\'e} du Foresto}, V.
	},
    title = "{Data reduction methods for single-mode optical interferometry. Application to the VLTI two-telescopes beam combiner VINCI}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0406625},
 keywords = {techniques: interferometric, methods: data analysis, instrumentation: interferometers},
     year = 2004,
    month = oct,
   volume = 425,
    pages = {1161-1174},
      doi = {10.1051/0004-6361:20034562},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...425.1161K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2003SPIE.4838..858K,
   author = {{Kervella}, P. and {Gitton}, P.~B. and {Segransan}, D. and {di Folco}, E. and 
	{Kern}, P.~Y. and {Kiekebusch}, M. and {Duc}, T.~P. and {Longinotti}, A. and 
	{Coud{\'e} du Foresto}, V. and {Ballester}, P. and {Sabet}, C. and 
	{Cotton}, W.~D. and {Schoeller}, M. and {Wilhelm}, R.},
    title = "{VINCI, the VLTI commissioning instrument: status after one year of operations at Paranal}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2003,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 4838,
   editor = "{W.~A.~Traub}",
    month = feb,
    pages = {858-869},
   adsurl = {http://adsabs.harvard.edu/abs/2003SPIE.4838..858K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2008PASP..120..617V,
   author = {{van Belle}, G.~T.},
    title = "{Closure Phase Signatures of Planet Transit Events}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {0804.2674},
 keywords = {Extrasolar Planets},
     year = 2008,
    month = may,
   volume = 120,
    pages = {617-624},
      doi = {10.1086/589310},
   adsurl = {http://adsabs.harvard.edu/abs/2008PASP..120..617V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2008SPIE.7013E..91R,
   author = {{Renard}, S. and {Absil}, O. and {Berger}, {J.-P.} and {Bonfils}, X. and 
	{Forveille}, T. and {Malbet}, F.},
    title = "{Prospects for near-infrared characterisation of hot Jupiters with the VLTI Spectro-Imager (VSI)}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2008,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 7013,
archivePrefix = "arXiv",
   eprint = {0807.3014},
    month = jul,
      doi = {10.1117/12.790494},
   adsurl = {http://adsabs.harvard.edu/abs/2008SPIE.7013E..91R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007NewAR..51..604M,
   author = {{Monnier}, J.~D.},
    title = "{Phases in interferometry}",
  journal = {New Astronomy Review},
     year = 2007,
    month = oct,
   volume = 51,
    pages = {604-616},
      doi = {10.1016/j.newar.2007.06.006},
   adsurl = {http://adsabs.harvard.edu/abs/2007NewAR..51..604M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007A&A...464....1P,
   author = {{Petrov}, R.~G. and {Malbet}, F. and {Weigelt}, G. and {Antonelli}, P. and 
	{Beckmann}, U. and {Bresson}, Y. and {Chelli}, A. and {Dugu{\'e}}, M. and 
	{Duvert}, G. and {Gennari}, S. and {Gl{\"u}ck}, L. and {Kern}, P. and 
	{Lagarde}, S. and {Le Coarer}, E. and {Lisi}, F. and {Millour}, F. and 
	{Perraut}, K. and {Puget}, P. and {Rantakyr{\"o}}, F. and {Robbe-Dubois}, S. and 
	{Roussel}, A. and {Salinari}, P. and {Tatulli}, E. and {Zins}, G. and 
	{Accardo}, M. and {Acke}, B. and {Agabi}, K. and {Altariba}, E. and 
	{Arezki}, B. and {Aristidi}, E. and {Baffa}, C. and {Behrend}, J. and 
	{Bl{\"o}cker}, T. and {Bonhomme}, S. and {Busoni}, S. and {Cassaing}, F. and 
	{Clausse}, J.-M. and {Colin}, J. and {Connot}, C. and {Delboulb{\'e}}, A. and 
	{Domiciano de Souza}, A. and {Driebe}, T. and {Feautrier}, P. and 
	{Ferruzzi}, D. and {Forveille}, T. and {Fossat}, E. and {Foy}, R. and 
	{Fraix-Burnet}, D. and {Gallardo}, A. and {Giani}, E. and {Gil}, C. and 
	{Glentzlin}, A. and {Heiden}, M. and {Heininger}, M. and {Hernandez Utrera}, O. and 
	{Hofmann}, K.-H. and {Kamm}, D. and {Kiekebusch}, M. and {Kraus}, S. and 
	{Le Contel}, D. and {Le Contel}, J.-M. and {Lesourd}, T. and 
	{Lopez}, B. and {Lopez}, M. and {Magnard}, Y. and {Marconi}, A. and 
	{Mars}, G. and {Martinot-Lagarde}, G. and {Mathias}, P. and 
	{M{\`e}ge}, P. and {Monin}, J.-L. and {Mouillet}, D. and {Mourard}, D. and 
	{Nussbaum}, E. and {Ohnaka}, K. and {Pacheco}, J. and {Perrier}, C. and 
	{Rabbia}, Y. and {Rebattu}, S. and {Reynaud}, F. and {Richichi}, A. and 
	{Robini}, A. and {Sacchettini}, M. and {Schertl}, D. and {Sch{\"o}ller}, M. and 
	{Solscheid}, W. and {Spang}, A. and {Stee}, P. and {Stefanini}, P. and 
	{Tallon}, M. and {Tallon-Bosc}, I. and {Tasso}, D. and {Testi}, L. and 
	{Vakili}, F. and {von der L{\"u}he}, O. and {Valtier}, J.-C. and 
	{Vannier}, M. and {Ventura}, N.},
    title = "{AMBER, the near-infrared spectro-interferometric three-telescope VLTI instrument}",
  journal = {\aap},
 keywords = {instrumentation: high angular resolution, techniques:, interferometric, techniques: spectroscopic},
     year = 2007,
    month = mar,
   volume = 464,
    pages = {1-12},
      doi = {10.1051/0004-6361:20066496},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...464....1P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2000SPIE.4006..407L,
   author = {{Lopez}, B. and {Petrov}, R.~G. and {Vannier}, M.},
    title = "{Direct detection of hot extrasolar planets with the VLTI using differential interferometry}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2000,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 4006,
   editor = "{P.~L{\'e}na \& A.~Quirrenbach}",
    month = jul,
    pages = {407-411},
   adsurl = {http://adsabs.harvard.edu/abs/2000SPIE.4006..407L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{2000SPIE.4006..269S,
   author = {{Segransan}, D. and {Beuzit}, J.-L. and {Delfosse}, X. and {Forveille}, T. and 
	{Mayor}, M. and {Perrier-Bellet}, C. and {Allard}, F.},
    title = "{How AMBER will contribute to the search for brown dwarfs and extrasolar giant planets}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2000,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 4006,
   editor = "{P.~L{\'e}na \& A.~Quirrenbach}",
    month = jul,
    pages = {269-276},
   adsurl = {http://adsabs.harvard.edu/abs/2000SPIE.4006..269S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{nordlund90,
   author = {{Nordlund}, A. and {Dravins}, D.},
    title = "{Stellar granulation. III - Hydrodynamic model atmospheres. IV - Line formation in inhomogeneous stellar photospheres. V - Synthetic spectral lines in disk-integrated starlight}",
  journal = {\aap},
 keywords = {ASTRONOMICAL MODELS, HYDRODYNAMICS, LATE STARS, SOLAR GRANULATION, STELLAR ATMOSPHERES, F STARS, G STARS, RADIATIVE TRANSFER, STELLAR MAGNETIC FIELDS, STELLAR TEMPERATURE, SUBGIANT STARS},
     year = 1990,
    month = feb,
   volume = 228,
    pages = {155-217},
   adsurl = {http://adsabs.harvard.edu/abs/1990A%26A...228..155N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mosser08,
   author = {{Mosser}, B. and {Bouchy}, F. and {Marti{\'c}}, M. and {Appourchaux}, T. and 
	{Barban}, C. and {Berthomieu}, G. and {Garcia}, R.~A. and {Lebrun}, J.~C. and 
	{Michel}, E. and {Provost}, J. and {Th{\'e}venin}, F. and {Turck-Chi{\`e}ze}, S.
	},
    title = "{Asteroseismology of Procyon with SOPHIE}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0712.1368},
 keywords = {techniques: radial velocities, stars: oscillations, stars: individual: {$\alpha$} CMi},
     year = 2008,
    month = jan,
   volume = 478,
    pages = {197-202},
      doi = {10.1051/0004-6361:20078337},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...478..197M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{belkacem11,
   author = {{Belkacem}, K. and {Goupil}, M.~J. and {Dupret}, M.~A. and {Samadi}, R. and 
    {Baudin}, F. and {Noels}, A. and {Mosser}, B.},
    title = "{The underlying physical meaning of the {$\nu$}$_{max}$ - {$\nu$}$_{c}$ relation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1104.0630},
 primaryClass = "astro-ph.SR",
 keywords = {convection, turbulence, stars: oscillations, stars: interiors},
     year = 2011,
    month = jun,
   volume = 530,
      eid = {A142},
    pages = {A142},
      doi = {10.1051/0004-6361/201116490},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...530A.142B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chollet99,
   author = {{Chollet}, F. and {Sinceac}, V.},
    title = "{Analysis of solar radius determination obtained by the modern CCD astrolabe of the Calern Observatory. A new approach of the solar limb definition}",
  journal = {\aaps},
 keywords = {SUN: GENERAL, SUN: OSCILLATIONS, SUN: PHOTOSPHERE, SUN: RADIUS, ASTROMETRY, ATMOSPHERIC EFFECTS},
     year = 1999,
    month = oct,
   volume = 139,
    pages = {219-229},
      doi = {10.1051/aas:1999507},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26AS..139..219C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{matthews04,
   author = {{Matthews}, J.~M. and {Kuschnig}, R. and {Guenther}, D.~B. and 
    {Walker}, G.~A.~H. and {Moffat}, A.~F.~J. and {Rucinski}, S.~M. and 
    {Sasselov}, D. and {Weiss}, W.~W.},
    title = "{No stellar p-mode oscillations in space-based photometry of Procyon}",
  journal = {\nat},
     year = 2004,
    month = jul,
   volume = 430,
    pages = {51-53},
      doi = {10.1038/nature02671},
   adsurl = {http://adsabs.harvard.edu/abs/2004Natur.430...51M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanleeuwen07,
   author = {{van Leeuwen}, F.},
    title = "{Validation of the new Hipparcos reduction}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0708.1752},
 keywords = {space vehicles: instruments, methods: data analysis, catalogs,
astrometry, instrumentation: miscellaneous},
     year = 2007,
    month = nov,
   volume = 474,
    pages = {653-664},
      doi = {10.1051/0004-6361:20078357},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...474..653V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fuhrmann97,
   author = {{Fuhrmann}, K. and {Pfeiffer}, M. and {Frank}, C. and {Reetz}, J. and 
    {Gehren}, T.},
    title = "{The surface gravities of cool dwarf stars revisited.}",
  journal = {\aap},
 keywords = {TECHNIQUES: SPECTROSCOPIC, STARS: FUNDAMENTAL PARAMETERS, STARS: INDIVIDUAL: PROCYON, STARS: LATE-TYPE, STARS: SUBDWARFS, GALAXY: EVOLUTION},
     year = 1997,
    month = jul,
   volume = 323,
    pages = {909-922},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...323..909F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{steffen85,
   author = {{Steffen}, M.},
    title = "{A model atmosphere analysis of the F5 IV-V subgiant Procyon}",
  journal = {\aaps},
 keywords = {BINARY STARS, STELLAR ATMOSPHERES, STELLAR COMPOSITION, STELLAR MODELS, STELLAR SPECTRA, SUBGIANT STARS, ABUNDANCE, SPECTRAL LINE WIDTH, STELLAR MASS, STELLAR TEMPERATURE, WHITE DWARF STARS},
     year = 1985,
    month = mar,
   volume = 59,
    pages = {403-427},
   adsurl = {http://adsabs.harvard.edu/abs/1985A%26AS...59..403S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{eggen65,
   author = {{Eggen}, O.~J. and {Greenstein}, J.~L.},
    title = "{Spectra, colors, luminosities, and motions of the white dwarfs}",
  journal = {\apj},
     year = 1965,
    month = jan,
   volume = 141,
    pages = {83},
      doi = {10.1086/148091},
   adsurl = {http://adsabs.harvard.edu/abs/1965ApJ...141...83E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{auwers1862,
   author = {{Auwers}, G.~F.~J.~A.},
    title = "{De motu proprio Procyonis variabili ...}",
 keywords = {SUAR: PROPER MOTION},
booktitle = {Regimonti Prussorum, typis academicis Dalkowskianis, 1862.},
     year = 1862,
   editor = "{Auwers, G.~F.~J.~A.}",
   adsurl = {http://adsabs.harvard.edu/abs/1862QB811.A94......},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{blackwell80,
   author = {{Blackwell}, D.~E. and {Petford}, A.~D. and {Shallis}, M.~J.
	},
    title = "{Use of the infra-red flux method for determining stellar effective temperatures and angular diameters - The stellar temperature scale}",
  journal = {\aap},
 keywords = {ATMOSPHERIC MODELS, DIAMETERS, INFRARED ASTRONOMY, STELLAR ATMOSPHERES, STELLAR TEMPERATURE, TEMPERATURE SCALES, INFRARED RADIATION, RADIANT FLUX DENSITY, STELLAR LUMINOSITY, STELLAR SPECTRA},
     year = 1980,
    month = feb,
   volume = 82,
    pages = {249-252},
   adsurl = {http://adsabs.harvard.edu/abs/1980A%26A....82..249B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...633..424A,
   author = {{Aufdenberg}, J.~P. and {Ludwig}, H.-G. and {Kervella}, P.},
    title = "{On the Limb Darkening, Spectral Energy Distribution, and Temperature Structure of Procyon}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0507336},
 keywords = {Convection, Methods: Numerical, Stars: Atmospheres, stars: fundamental parameters (colors), stars: fundamental parameters (temperatures), Stars: Individual: Name: Procyon, Techniques: Interferometric},
     year = 2005,
    month = nov,
   volume = 633,
    pages = {424-439},
      doi = {10.1086/452622},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...633..424A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...528A.120C,
   author = {{Chiavassa}, A. and {Pasquato}, E. and {Jorissen}, A. and {Sacuto}, S. and 
	{Babusiaux}, C. and {Freytag}, B. and {Ludwig}, H.-G. and {Cruzal{\`e}bes}, P. and 
	{Rabbia}, Y. and {Spang}, A. and {Chesneau}, O.},
    title = "{Radiative hydrodynamic simulations of red supergiant stars. III. Spectro-photocentric variability, photometric variability, and consequences on Gaia measurements}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1012.5234},
 primaryClass = "astro-ph.SR",
 keywords = {stars: atmospheres, supergiants, astrometry, parallaxes, hydrodynamics, stars: individual: Betelgeuse},
     year = 2011,
    month = apr,
   volume = 528,
    pages = {A120 },
      doi = {10.1051/0004-6361/201015768},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...528A.120C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992A&AS...92....1G,
   author = {{Glushneva}, I.~N. and {Kharitonov}, A.~V. and {Kniazeva}, L.~N. and 
	{Shenavrin}, V.~I.},
    title = "{Secondary spectrophotometric standards}",
  journal = {\aaps},
 keywords = {ASTRONOMICAL CATALOGS, SPECTRAL ENERGY DISTRIBUTION, STANDARDS, STELLAR SPECTROPHOTOMETRY, INFRARED SPECTROSCOPY, NEAR INFRARED RADIATION},
     year = 1992,
    month = jan,
   volume = 92,
    pages = {1-29},
   adsurl = {http://adsabs.harvard.edu/abs/1992A%26AS...92....1G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999A&AS..139..183R,
   author = {{Rodr{\'{\i}}guez-Pascual}, P.~M. and {Gonz{\'a}lez-Riestra}, R. and 
	{Schartel}, N. and {Wamsteker}, W.},
    title = "{The IUE INES System: Improved data extraction procedures for IUE}",
  journal = {\aaps},
 keywords = {METHODS: DATA ANALYSIS, SPACE VEHICLES, TECHNIQUES: IMAGE PROCESSING, ULTRAVIOLET: GENERAL},
     year = 1999,
    month = oct,
   volume = 139,
    pages = {183-197},
      doi = {10.1051/aas:1999388},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26AS..139..183R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1955VA......1..249U,
   author = {{Uns{\"o}ld}, A. and {Weidemann}, V.},
    title = "{Fraunhofer lines and the structure of stellar atmospheres}",
  journal = {Vistas in Astronomy},
     year = 1955,
   volume = 1,
    pages = {249-256},
      doi = {10.1016/0083-6656(55)90033-7},
   adsurl = {http://adsabs.harvard.edu/abs/1955VA......1..249U},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998A&A...333..231B,
   author = {{Bessell}, M.~S. and {Castelli}, F. and {Plez}, B.},
    title = "{Model atmospheres broad-band colors, bolometric corrections and temperature calibrations for O - M stars}",
  journal = {\aap},
 keywords = {STARS: ATMOSPHERES, FUNDAMENTAL PARAMETERS, GENERAL},
     year = 1998,
    month = may,
   volume = 333,
    pages = {231-250},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...333..231B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1990PASP..102.1181B,
   author = {{Bessell}, M.~S.},
    title = "{UBVRI passbands}",
  journal = {\pasp},
 keywords = {ASTRONOMICAL PHOTOMETRY, SPECTRAL BANDS, UBV SPECTRA, CHARGE COUPLED DEVICES, REFERENCE STARS, STELLAR COLOR, STELLAR MAGNITUDE},
     year = 1990,
    month = oct,
   volume = 102,
    pages = {1181-1199},
      doi = {10.1086/132749},
   adsurl = {http://adsabs.harvard.edu/abs/1990PASP..102.1181B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2003AJ....126.1090C,
   author = {{Cohen}, M. and {Wheaton}, W.~A. and {Megeath}, S.~T.},
    title = "{Spectral Irradiance Calibration in the Infrared. XIV. The Absolute Calibration of 2MASS}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/0304350},
 keywords = {Infrared Radiation, Surveys},
     year = 2003,
    month = aug,
   volume = 126,
    pages = {1090-1096},
      doi = {10.1086/376474},
   adsurl = {http://adsabs.harvard.edu/abs/2003AJ....126.1090C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...530..307C,
   author = {{Carr}, J.~S. and {Sellgren}, K. and {Balachandran}, S.~C.},
    title = "{The First Stellar Abundance Measurements in the Galactic Center: The M Supergiant IRS 7}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9909037},
 keywords = {GALAXY: CENTER, STARS: ABUNDANCES, STARS: LATE-TYPE, STARS: SUPERGIANTS},
     year = 2000,
    month = feb,
   volume = 530,
    pages = {307-322},
      doi = {10.1086/308340},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...530..307C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1990MNRAS.245P...7B,
   author = {{Buscher}, D.~F. and {Baldwin}, J.~E. and {Warner}, P.~J. and 
	{Haniff}, C.~A.},
    title = "{Detection of a bright feature on the surface of Betelgeuse}",
  journal = {\mnras},
     year = 1990,
    month = jul,
   volume = 245,
    pages = {7P-11P},
   adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.245P...7B},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}


@ARTICLE{1997MNRAS.285..529T,
   author = {{Tuthill}, P.~G. and {Haniff}, C.~A. and {Baldwin}, J.~E.},
    title = "{Hotspots on late-type supergiants}",
  journal = {\mnras},
 keywords = {STARS, IMAGING: STARS, INDIVIDUAL, ALPHA ORI: STARS, INDIVIDUAL, ALPHA HER: STARS, INDIVIDUAL, ALPHA SCO: SUPERGIANTS},
     year = 1997,
    month = mar,
   volume = 285,
    pages = {529-539},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.285..529T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...529A.163O,
   author = {{Ohnaka}, K. and {Weigelt}, G. and {Millour}, F. and {Hofmann}, K.-H. and 
	{Driebe}, T. and {Schertl}, D. and {Chelli}, A. and {Massi}, F. and 
	{Petrov}, R. and {Stee}, P.},
    title = "{Imaging the dynamical atmosphere of the red supergiant Betelgeuse in the CO first overtone lines with VLTI/AMBER}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1104.0958},
 primaryClass = "astro-ph.SR",
 keywords = {infrared: stars, techniques: interferometric, supergiants, stars: late-type, stars: atmospheres, stars: individual: Betelgeuse},
     year = 2011,
    month = may,
   volume = 529,
    pages = {A163 },
      doi = {10.1051/0004-6361/201016279},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...529A.163O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2009A&A...503..183O,
   author = {{Ohnaka}, K. and {Hofmann}, {K.-H.} and {Benisty}, M. and {Chelli}, A. and 
	{Driebe}, T. and {Millour}, F. and {Petrov}, R. and {Schertl}, D. and 
	{Stee}, P. and {Vakili}, F. and {Weigelt}, G.},
    title = "{Spatially resolving the inhomogeneous structure of the dynamical atmosphere of Betelgeuse with VLTI/AMBER}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0906.4792},
 keywords = {infrared: stars, techniques: interferometric, stars: supergiants, stars: late-type, stars: atmospheres, stars: individual: Betelgeuse},
     year = 2009,
    month = aug,
   volume = 503,
    pages = {183-195},
      doi = {10.1051/0004-6361/200912247},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...503..183O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000MNRAS.315..635Y,
   author = {{Young}, J.~S. and {Baldwin}, J.~E. and {Boysen}, R.~C. and 
	{Haniff}, C.~A. and {Lawson}, P.~R. and {Mackay}, C.~D. and 
	{Pearson}, D. and {Rogers}, J. and {St.-Jacques}, D. and {Warner}, P.~J. and 
	{Wilson}, D.~M.~A. and {Wilson}, R.~W.},
    title = "{New views of Betelgeuse: multi-wavelength surface imaging and implications for models of hotspot generation}",
  journal = {\mnras},
     year = 2000,
    month = jul,
   volume = 315,
    pages = {635-645},
   adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.315..635Y},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{2000MNRAS.315..635Y,
   author = {{Young}, J.~S. and {Baldwin}, J.~E. and {Boysen}, R.~C. and 
	{Haniff}, C.~A. and {Lawson}, P.~R. and {Mackay}, C.~D. and 
	{Pearson}, D. and {Rogers}, J. and {St.-Jacques}, D. and {Warner}, P.~J. and 
	{Wilson}, D.~M.~A. and {Wilson}, R.~W.},
    title = "{New views of Betelgeuse: multi-wavelength surface imaging and implications for models of hotspot generation}",
  journal = {\mnras},
     year = 2000,
    month = jul,
   volume = 315,
    pages = {635-645},
   adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.315..635Y},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...508..923H,
   author = {{Haubois}, X. and {Perrin}, G. and {Lacour}, S. and {Verhoelst}, T. and 
	{Meimon}, S. and {Mugnier}, L. and {Thi{\'e}baut}, E. and {Berger}, J.~P. and 
	{Ridgway}, S.~T. and {Monnier}, J.~D. and {Millan-Gabet}, R. and 
	{Traub}, W.},
    title = "{Imaging the spotty surface of <ASTROBJ>Betelgeuse</ASTROBJ> in the H band}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0910.4167},
 keywords = {convection, techniques: interferometric, stars: fundamental parameters, infrared: stars, stars: individual: <ASTROBJ>Betelgeuse</ASTROBJ>},
     year = 2009,
    month = dec,
   volume = 508,
    pages = {923-932},
      doi = {10.1051/0004-6361/200912927},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...508..923H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...504..115K,
   author = {{Kervella}, P. and {Verhoelst}, T. and {Ridgway}, S.~T. and 
	{Perrin}, G. and {Lacour}, S. and {Cami}, J. and {Haubois}, X.
	},
    title = "{The close circumstellar environment of Betelgeuse. Adaptive optics spectro-imaging in the near-IR with VLT/NACO}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0907.1843},
 keywords = {stars: individual: Betelgeuse, stars: imaging, stars: supergiants, stars: circumstellar matter, methods: observational , techniques: high angular resolution},
     year = 2009,
    month = sep,
   volume = 504,
    pages = {115-125},
      doi = {10.1051/0004-6361/200912521},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...504..115K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992MNRAS.257..369W,
   author = {{Wilson}, R.~W. and {Baldwin}, J.~E. and {Buscher}, D.~F. and 
	{Warner}, P.~J.},
    title = "{High-resolution imaging of Betelgeuse and Mira}",
  journal = {\mnras},
 keywords = {ASTRONOMICAL PHOTOGRAPHY, BRIGHTNESS DISTRIBUTION, GIANT STARS, HIGH RESOLUTION, MIRA VARIABLES, SUPERGIANT STARS, CHARGE COUPLED DEVICES, COMPANION STARS, INTERFEROMETRY, LIMB DARKENING, PHOTOSPHERE, POWER SPECTRA},
     year = 1992,
    month = aug,
   volume = 257,
    pages = {369-376},
   adsurl = {http://adsabs.harvard.edu/abs/1992MNRAS.257..369W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997MNRAS.291..819W,
   author = {{Wilson}, R.~W. and {Dhillon}, V.~S. and {Haniff}, C.~A.},
    title = "{The changing face of Betelgeuse}",
  journal = {\mnras},
     year = 1997,
    month = nov,
   volume = 291,
    pages = {819},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.291..819W},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2004young,
   author = {{Young}, J.~S. and {Badsen}, A.~G. and {Bharmal}, N.~A. and {Boysen}, R.~C. and {O'Donova}, B. and {Seneta}, E.~B. and {Thorsteinsson}, H. and 
	{Thureau}, N.~D. and {Pedretti}, E. and {Monnier}, J.~D.},
    title = "{Unveling Alpha Orionis}",
  journal = {UK National Astronomy Meeting},
     year = 2004,
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...504..115K,
   author = {{Kervella}, P. and {Verhoelst}, T. and {Ridgway}, S.~T. and 
	{Perrin}, G. and {Lacour}, S. and {Cami}, J. and {Haubois}, X.
	},
    title = "{The close circumstellar environment of Betelgeuse. Adaptive optics spectro-imaging in the near-IR with VLT/NACO}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0907.1843},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: Betelgeuse, stars: imaging, stars: supergiants, stars: circumstellar matter, methods: observational , techniques: high angular resolution},
     year = 2009,
    month = sep,
   volume = 504,
    pages = {115-125},
      doi = {10.1051/0004-6361/200912521},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...504..115K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000A&A...357..225J,
   author = {{Josselin}, E. and {Blommaert}, J.~A.~D.~L. and {Groenewegen}, M.~A.~T. and 
	{Omont}, A. and {Li}, F.~L.},
    title = "{Observational investigation of mass loss of M supergiants}",
  journal = {\aap},
 keywords = {STARS: CIRCUMSTELLAR MATTER, STARS: MASS-LOSS, STARS: SUPERGIANTS, INFRARED: STARS},
     year = 2000,
    month = may,
   volume = 357,
    pages = {225-232},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...357..225J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006ApJ...645.1102L,
   author = {{Levesque}, E.~M. and {Massey}, P. and {Olsen}, K.~A.~G. and
        {Plez}, B. and {Meynet}, G. and {Maeder}, A.},
    title = "{The Effective Temperatures and Physical Properties of Magellanic Cloud Red Supergiants: The Effects of Metallicity}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0603596},
 keywords = {ISM: Dust, Extinction, Stars: Atmospheres, Stars: Fundamental Parameters, Stars: Late-Type, Stars: Supergiants},
     year = 2006,
    month = jul,
   volume = 645,
    pages = {1102-1117},
      doi = {10.1086/504417},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006ApJ...645.1102L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...660..301M,
   author = {{Massey}, P. and {Levesque}, E.~M. and {Olsen}, K.~A.~G. and
        {Plez}, B. and {Skiff}, B.~A.},
    title = "{HV 11423: The Coolest Supergiant in the SMC}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0701769},
 keywords = {Stars: Atmospheres, Stars: Evolution, Stars: Late-Type, Stars: Supergiants},
     year = 2007,
    month = may,
   volume = 660,
    pages = {301-310},
      doi = {10.1086/513182},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007ApJ...660..301M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...667..202L,
   author = {{Levesque}, E.~M. and {Massey}, P. and {Olsen}, K.~A.~G. and
        {Plez}, B.},
    title = "{Late-Type Red Supergiants: Too Cool for the Magellanic Clouds?}",
  journal = {\apj},
   eprint = {arXiv:0705.3431},
 keywords = {Stars: Evolution, Stars: Late-Type, Stars: Mass Loss, Stars: Supergiants},
     year = 2007,
    month = sep,
   volume = 667,
    pages = {202-212},
      doi = {10.1086/520797},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007ApJ...667..202L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2010NewAR..54....1L,
   author = {{Levesque}, E.~M.},
    title = "{The physical properties of red supergiants}",
  journal = {\nar},
archivePrefix = "arXiv",
   eprint = {0911.4720},
 primaryClass = "astro-ph.SR",
     year = 2010,
    month = jan,
   volume = 54,
    pages = {1-12},
      doi = {10.1016/j.newar.2009.10.002},
   adsurl = {http://adsabs.harvard.edu/abs/2010NewAR..54....1L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...516L...2A,
   author = {{Auri{\`e}re}, M. and {Donati}, {J.-F.} and {Konstantinova-Antova}, R. and 
	{Perrin}, G. and {Petit}, P. and {Roudier}, T.},
    title = "{The magnetic field of Betelgeuse: a local dynamo from giant convection cells?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1005.4845},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: Betelgeuse, stars: magnetic field, stars: late-type, supergiants},
     year = 2010,
    month = jun,
   volume = 516,
    pages = {L2},
      doi = {10.1051/0004-6361/201014925},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...516L...2A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984ApJ...284..238H,
   author = {{Hartmann}, L. and {Avrett}, E.~H.},
    title = "{On the extended chromosphere of Alpha Orionis}",
  journal = {\apj},
 keywords = {CHROMOSPHERE, M STARS, STELLAR MASS EJECTION, SUPERGIANT STARS, BRIGHTNESS DISTRIBUTION, RADIO EMISSION, STELLAR MODELS, STELLAR SPECTRA, STELLAR WINDS},
     year = 1984,
    month = sep,
   volume = 284,
    pages = {238-249},
      doi = {10.1086/162402},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...284..238H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989A&A...209..198P,
   author = {{Pijpers}, F.~P. and {Hearn}, A.~G.},
    title = "{A model for a stellar wind driven by linear acoustic waves}",
  journal = {\aap},
 keywords = {COMPUTATIONAL ASTROPHYSICS, SOUND WAVES, STELLAR MODELS, STELLAR OSCILLATIONS, STELLAR WINDS, MASS TRANSFER, MOMENTUM TRANSFER, STELLAR CORONAS, STELLAR MASS EJECTION},
     year = 1989,
    month = jan,
   volume = 209,
    pages = {198-210},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...209..198P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997A&A...325..709C,
   author = {{Cuntz}, M.},
    title = "{Chromospheric velocity fields in {$\alpha$} Orionis (M2 Iab) generated by stochastic shocks.}",
  journal = {\aap},
 keywords = {HYDRODYNAMICS, SHOCK WAVES, WAVES, STARS: CHROMOSPHERES, STARS: INDIVIDUAL: $\{$ALPHA$\}$ ORI, STARS: SUPERGIANTS},
     year = 1997,
    month = sep,
   volume = 325,
    pages = {709-713},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...325..709C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2010MNRAS.408.2290G,
   author = {{Grunhut}, J.~H. and {Wade}, G.~A. and {Hanes}, D.~A. and {Alecian}, E.
	},
    title = "{Systematic detection of magnetic fields in massive, late-type supergiants}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1006.5891},
 primaryClass = "astro-ph.SR",
 keywords = {techniques: polarimetric, techniques: spectropolarimetry, stars: late-type, stars: magnetic field, stars: massive, stars: supergiants},
     year = 2010,
    month = nov,
   volume = 408,
    pages = {2290-2297},
      doi = {10.1111/j.1365-2966.2010.17275.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.408.2290G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007A&A...469..671J,
   author = {{Josselin}, E. and {Plez}, B.},
    title = "{Atmospheric dynamics and the mass loss process in red supergiant stars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0705.0266},
 keywords = {supergiants, stars: atmospheres, stars: mass-loss},
     year = 2007,
    month = jul,
   volume = 469,
    pages = {671-680},
      doi = {10.1051/0004-6361:20066353},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..671J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2010A&A...511A..51C,
   author = {{Chiavassa}, A. and {Lacour}, S. and {Millour}, F. and {Driebe}, T. and 
	{Wittkowski}, M. and {Plez}, B. and {Thi{\'e}baut}, E. and {Josselin}, E. and 
	{Freytag}, B. and {Scholz}, M. and {Haubois}, X.},
    title = "{VLTI/AMBER spectro-interferometric imaging of VX Sagittarii's inhomogenous outer atmosphere}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0911.4422},
 primaryClass = "astro-ph.SR",
 keywords = {stars: AGB and post-AGB, stars: atmospheres, stars: individual: VX Sagittarii, techniques: interferometric, supergiants},
     year = 2010,
    month = feb,
   volume = 511,
    pages = {A51 },
      doi = {10.1051/0004-6361/200913288},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...511A..51C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1999A&A...346L..17A,
   author = {{Asplund}, M. and {Nordlund}, {\AA}. and {Trampedach}, R. and 
	{Stein}, R.~F.},
    title = "{3D hydrodynamical model atmospheres of metal-poor stars. Evidence for a low primordial Li abundance}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/9905059},
 keywords = {CONVECTION, STARS: ABUNDANCES, STARS: ATMOSPHERES, STARS: POPULATION II, LINE: FORMATION},
     year = 1999,
    month = jun,
   volume = 346,
    pages = {L17-L20},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...346L..17A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001A&A...372..601A,
   author = {{Asplund}, M. and {Garc{\'{\i}}a P{\'e}rez}, A.~E.},
    title = "{On OH line formation and oxygen abundances in metal-poor stars}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0104071},
 keywords = {CONVECTION, LINE: FORMATION, STARS: ABUNDANCES, STARS: ATMOSPHERES, STARS: POPULATION II, GALAXY: EVOLUTION},
     year = 2001,
    month = jun,
   volume = 372,
    pages = {601-615},
      doi = {10.1051/0004-6361:20010483},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...372..601A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ARA&A..47..481A,
   author = {{Asplund}, M. and {Grevesse}, N. and {Sauval}, A.~J. and {Scott}, P.
	},
    title = "{The Chemical Composition of the Sun}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0909.0948},
     year = 2009,
    month = sep,
   volume = 47,
    pages = {481-522},
      doi = {10.1146/annurev.astro.46.060407.145222},
   adsurl = {http://adsabs.harvard.edu/abs/2009ARA%26A..47..481A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2009MmSAI..80..711L,
   author = {{Ludwig}, {H.-G.} and {Caffau}, E. and {Steffen}, M. and {Freytag}, B. and 
	{Bonifacio}, P. and {Ku{\v c}inskas}, A.},
    title = "{The CIFIST 3D model atmosphere grid.}",
  journal = {\memsai},
archivePrefix = "arXiv",
   eprint = {0908.4496},
 primaryClass = "astro-ph.SR",
 keywords = {Stars: abundances, Stars: atmospheres, hydrodynamics, convection, radiative transfer},
     year = 2009,
   volume = 80,
    pages = {711- },
   adsurl = {http://adsabs.harvard.edu/abs/2009MmSAI..80..711L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989A&A...213..371S,
   author = {{Steffen}, M. and {Ludwig}, H.-G. and {Kruess}, A.},
    title = "{A numerical simulation study of solar granular convection in cells of different horizontal dimension}",
  journal = {\aap},
     year = 1989,
    month = apr,
   volume = 213,
    pages = {371-382},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...213..371S},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{2000SoPh..192...91S,
   author = {{Stein}, R.~F. and {Nordlund}, {\AA}.},
    title = "{Realistic Solar Convection Simulations}",
  journal = {\solphys},
     year = 2000,
    month = mar,
   volume = 192,
    pages = {91-108},
   adsurl = {http://adsabs.harvard.edu/abs/2000SoPh..192...91S},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1992iesh.conf...86G,
   author = {{Gustafsson}, B. and {Plez}, B.},
    title = "{Can classical model atmospheres be of any use for the study of hypergiants}",
booktitle = {Instabilities in Evolved Super- and Hypergiants},
     year = 1992,
   editor = "{C.~de Jager \& H.~Nieuwenhuijzen}",
    pages = {86},
   adsurl = {http://adsabs.harvard.edu/abs/1992iesh.conf...86G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2005ApJ...634.1286M,
   author = {{Massey}, P. and {Plez}, B. and {Levesque}, E.~M. and {Olsen}, K.~A.~G. and 
	{Clayton}, G.~C. and {Josselin}, E.},
    title = "{The Reddening of Red Supergiants: When Smoke Gets in Your Eyes}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0508254},
 keywords = {ISM: Dust, Extinction, Stars: Atmospheres, Stars: Fundamental Parameters, Stars: Late-Type, Stars: Supergiants},
     year = 2005,
    month = dec,
   volume = 634,
    pages = {1286-1292},
      doi = {10.1086/497065},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634.1286M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1993ApJ...418..812P,
   author = {{Plez}, B. and {Smith}, V.~V. and {Lambert}, D.~L.},
    title = "{Lithium Abundances and Other Clues to Envelope Burning in Small Magellanic Cloud Asymptotic Giant Branch Stars}",
  journal = {\apj},
     year = 1993,
    month = dec,
   volume = 418,
    pages = {812},
      doi = {10.1086/173438},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...418..812P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998A&A...330.1109A,
   author = {{Alvarez}, R. and {Plez}, B.},
    title = "{Near-infrared narrow-band photometry of M-giant and Mira stars: models meet observations}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/9710157},
     year = 1998,
    month = feb,
   volume = 330,
    pages = {1109-1119},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...330.1109A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2009MmSAI..80..731S,
   author = {{Steffen}, M. and {Ludwig}, {H.-G.} and {Caffau}, E.},
    title = "{Micro- and macroturbulence derived from 3D hydrodynamical stellar atmospheres .}",
  journal = {\memsai},
archivePrefix = "arXiv",
   eprint = {0909.2831},
 primaryClass = "astro-ph.SR",
 keywords = {Sun: abundances, Stars: abundances, Hydrodynamics, Turbulence, Line: formation},
     year = 2009,
   volume = 80,
    pages = {731- },
   adsurl = {http://adsabs.harvard.edu/abs/2009MmSAI..80..731S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...513A..72B,
   author = {{Behara}, N.~T. and {Bonifacio}, P. and {Ludwig}, {H.-G.} and 
	{Sbordone}, L. and {Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and {Caffau}, E.
	},
    title = "{Three carbon-enhanced metal-poor dwarf stars from the SDSS. Chemical abundances from CO^{5}BOLD 3D hydrodynamical model atmospheres}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1002.1670},
 keywords = {stars: individual: SDSS J1349-0229, stars: individual: SDSS J0912 0216, stars: individual: SDSS J1036 1212, stars: abundances, stars: AGB and post-AGB, stars: atmospheres},
     year = 2010,
    month = apr,
   volume = 513,
    pages = {A72},
      doi = {10.1051/0004-6361/200913213},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...513A..72B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000A&A...359..669A,
   author = {{Asplund}, M. and {Ludwig}, {H.-G.} and {Nordlund}, {\AA}. and 
	{Stein}, R.~F.},
    title = "{The effects of numerical resolution on hydrodynamical surface convection simulations and spectral line formation}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0005319},
 keywords = {CONVECTION, HYDRODYNAMICS, LINE: FORMATION, SUN: ABUNDANCES, SUN: GRANULATION, SUN: PHOTOSPHERE},
     year = 2000,
    month = jul,
   volume = 359,
    pages = {669-681},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...359..669A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003MNRAS.340..923R,
   author = {{Robinson}, F.~J. and {Demarque}, P. and {Li}, L.~H. and {Sofia}, S. and 
	{Kim}, {Y.-C.} and {Chan}, K.~L. and {Guenther}, D.~B.},
    title = "{Three-dimensional convection simulations of the outer layers of the Sun using realistic physics}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0212296},
 keywords = {convection, methods: numerical, Sun: atmosphere, Sun: interior},
     year = 2003,
    month = apr,
   volume = 340,
    pages = {923-936},
      doi = {10.1046/j.1365-8711.2003.06349.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.340..923R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2003ASPC..293...64A,
   author = {{Asida}, S.~M.},
    title = "{Hydrodynamical Simulations of Convection Using 2D VULCAN}",
booktitle = {3D Stellar Evolution},
     year = 2003,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 293,
   editor = "{S.~Turcotte, S.~C.~Keller, \& R.~M.~Cavallo}",
    pages = {64},
   adsurl = {http://adsabs.harvard.edu/abs/2003ASPC..293...64A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...499..914S,
   author = {{Stein}, R.~F. and {Nordlund}, A.},
    title = "{Simulations of Solar Granulation. I. General Properties}",
  journal = {\apj},
 keywords = {METHODS: NUMERICAL, CONVECTION, SUN: GRANULATION, HYDRODYNAMICS, SUN: INTERIOR},
     year = 1998,
    month = may,
   volume = 499,
    pages = {914},
      doi = {10.1086/305678},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...499..914S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2010A&A...522A..26S,
   author = {{Sbordone}, L. and {Bonifacio}, P. and {Caffau}, E. and {Ludwig}, {H.-G.} and 
	{Behara}, N.~T. and {Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and 
	{Steffen}, M. and {Cayrel}, R. and {Freytag}, B. and {van't Veer}, C. and 
	{Molaro}, P. and {Plez}, B. and {Sivarani}, T. and {Spite}, M. and 
	{Spite}, F. and {Beers}, T.~C. and {Christlieb}, N. and {Fran{\c c}ois}, P. and 
	{Hill}, V.},
    title = "{The metal-poor end of the Spite plateau. I. Stellar parameters, metallicities, and lithium abundances}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1003.4510},
 primaryClass = "astro-ph.GA",
 keywords = {nuclear reactions, nucleosynthesis, abundances, Galaxy: halo, Galaxy: abundances, cosmology: observations, stars: Population II},
     year = 2010,
    month = nov,
   volume = 522,
    pages = {A26},
      doi = {10.1051/0004-6361/200913282},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...522A..26S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...508.1429W,
   author = {{Wende}, S. and {Reiners}, A. and {Ludwig}, {H.-G.}},
    title = "{3D simulations of M star atmosphere velocities and their influence on molecular FeH lines}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0910.3493},
 keywords = {hydrodynamics: stars: low-mass, brown dwarfs, line: profiles, turbulence, stars: late-type},
     year = 2009,
    month = dec,
   volume = 508,
    pages = {1429-1442},
      doi = {10.1051/0004-6361/200913149},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...508.1429W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009MmSAI..80..723K,
   author = {{Ku{\v c}inskas}, A. and {Ludwig}, {H.-G.} and {Caffau}, E. and 
	{Steffen}, M.},
    title = "{3D hydrodynamical simulations of stellar photospheres with the CO^{5}BOLD code. Photometric colors of a late-type giant}",
  journal = {Memorie della Societa Astronomica Italiana},
archivePrefix = "arXiv",
   eprint = {0910.3412},
 keywords = {Stars: late-type, Stars: atmospheres, Star: fundamental parameters, Physical data and processes: convection, Techniques: photometric},
     year = 2009,
   volume = 80,
    pages = {723- },
   adsurl = {http://adsabs.harvard.edu/abs/2009MmSAI..80..723K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...528A..32C,
   author = {{Collet}, R. and {Hayek}, W. and {Asplund}, M. and {Nordlund}, {\AA}. and 
	{Trampedach}, R. and {Gudiksen}, B.},
    title = "{Three-dimensional surface convection simulations of metal-poor stars. The effect of scattering on the photospheric temperature stratification}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1101.3265},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, convection, radiative transfer, scattering, stars: late-type, stars: atmospheres},
     year = 2011,
    month = apr,
   volume = 528,
    pages = {A32 },
      doi = {10.1051/0004-6361/201016151},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...528A..32C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2010SoPh..tmp...66C,
   author = {{Caffau}, E. and {Ludwig}, {H.-G.} and {Steffen}, M. and {Freytag}, B. and 
	{Bonifacio}, P.},
    title = "{Solar Chemical Abundances Determined with a CO5BOLD 3D Model Atmosphere}",
  journal = {\solphys},
archivePrefix = "arXiv",
   eprint = {1003.1190},
 keywords = {Sun: abundances, Sun: photosphere, Line: formation, Hydrodynamics, Convection, Radiative transfer},
     year = 2010,
    month = mar,
    pages = {66- },
      doi = {10.1007/s11207-010-9541-4},
   adsurl = {http://adsabs.harvard.edu/abs/2010SoPh..tmp...66C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2009MmSAI..80..719C,
   author = {{Collet}, R. and {Nordlund}, {\AA}. and {Asplund}, M. and {Hayek}, W. and 
	{Trampedach}, R.},
    title = "{Abundance analysis of the halo giant HD 122563 with three-dimensional model stellar atmospheres}",
  journal = {Memorie della Societa Astronomica Italiana},
archivePrefix = "arXiv",
   eprint = {0909.0690},
 keywords = {Convection, Hydrodynamics, Line: formation, Stars: abundances, Stars: atmospheres, Stars: late-type, Stars: individual: HD122563},
     year = 2009,
   volume = 80,
    pages = {719},
   adsurl = {http://adsabs.harvard.edu/abs/2009MmSAI..80..719C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2008AJ....135.1450G,
   author = {{Gray}, D.~F.},
    title = "{Mass Motions in the Photosphere of Betelgeuse}",
  journal = {\aj},
 keywords = {convection, stars: individual: Betelgeuse, stars: oscillations, stars: variables: other, supergiants, techniques: spectroscopic},
     year = 2008,
    month = apr,
   volume = 135,
    pages = {1450-1458},
      doi = {10.1088/0004-6256/135/4/1450},
   adsurl = {http://adsabs.harvard.edu/abs/2008AJ....135.1450G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1986A&A...163..135M,
   author = {{Magain}, P.},
    title = "{Contribution functions and the depths of formation of spectral lines}",
  journal = {\aap},
 keywords = {LINE SPECTRA, STELLAR ATMOSPHERES, STELLAR SPECTRA, ABSORPTION SPECTRA, IRON, PHOTOSPHERE, SPECTRAL LINE WIDTH, TRANSFER FUNCTIONS},
     year = 1986,
    month = jul,
   volume = 163,
    pages = {135-139},
   adsurl = {http://adsabs.harvard.edu/abs/1986A%26A...163..135M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2006EAS....18..177C,
   author = {{Chiavassa}, A. and {Plez}, B. and {Josselin}, E. and {Freytag}, B.
	},
    title = "{Radiative transfer in snapshots of 3D radiative hydrodynamic models of red supergiants}",
booktitle = {EAS Publications Series},
     year = 2006,
   series = {EAS Publications Series},
   volume = 18,
   editor = "{P.~Stee}",
    pages = {177-189},
      doi = {10.1051/eas:2006011},
   adsurl = {http://adsabs.harvard.edu/abs/2006EAS....18..177C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{barban99,
   author = {{Barban}, C. and {Michel}, E. and {Martic}, M. and {Schmitt}, J. and 
	{Lebrun}, J.~C. and {Baglin}, A. and {Bertaux}, J.~L.},
    title = "{Solar-like oscillations of Procyon A: stellar models and time series simulations versus observations}",
  journal = {\aap},
 keywords = {STARS: OSCILLATIONS, STARS: INDIVIDUAL: PROCYON A},
     year = 1999,
    month = oct,
   volume = 350,
    pages = {617-625},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...350..617B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{arentoft08,
   author = {{Arentoft}, T. and {Kjeldsen}, H. and {Bedding}, T.~R. and {Bazot}, M. and 
    {Christensen-Dalsgaard}, J. and {Dall}, T.~H. and {Karoff}, C. and 
    {Carrier}, F. and {Eggenberger}, P. and {Sosnowska}, D. and 
    {Wittenmyer}, R.~A. and {Endl}, M. and {Metcalfe}, T.~S. and 
    {Hekker}, S. and {Reffert}, S. and {Butler}, R.~P. and {Bruntt}, H. and 
    {Kiss}, L.~L. and {O'Toole}, S.~J. and {Kambe}, E. and {Ando}, H. and 
    {Izumiura}, H. and {Sato}, B. and {Hartmann}, M. and {Hatzes}, A. and 
    {Bouchy}, F. and {Mosser}, B. and {Appourchaux}, T. and {Barban}, C. and 
    {Berthomieu}, G. and {Garcia}, R.~A. and {Michel}, E. and {Provost}, J. and 
    {Turck-Chi{\`e}ze}, S. and {Marti{\'c}}, M. and {Lebrun}, J.-C. and 
    {Schmitt}, J. and {Bertaux}, J.-L. and {Bonanno}, A. and {Benatti}, S. and 
    {Claudi}, R.~U. and {Cosentino}, R. and {Leccia}, S. and {Frandsen}, S. and 
    {Brogaard}, K. and {Glowienka}, L. and {Grundahl}, F. and {Stempels}, E.
    },
    title = "{A Multisite Campaign to Measure Solar-like Oscillations in Procyon. I. Observations, Data Reduction, and Slow Variations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0807.3794},
 keywords = {Stars: Individual: Name: Procyon A, Stars: Oscillations},
     year = 2008,
    month = nov,
   volume = 687,
    pages = {1180-1190},
      doi = {10.1086/592040},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...687.1180A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kjeldsen95,
   author = {{Kjeldsen}, H. and {Bedding}, T.~R.},
    title = "{Amplitudes of stellar oscillations: the implications for asteroseismology.}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/9403015},
 keywords = {SUN: OSCILLATIONS, STARS: INDIVIDUAL: $\{$ALPHA$\}$ CEN, STARS: INDIVIDUAL: PROCYON, STARS: OSCILLATIONS, CEPHEIDS, $\{$DELTA$\}$ SCT},
     year = 1995,
    month = jan,
   volume = 293,
    pages = {87-106},
   adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...293...87K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kjeldsen11,
   author = {{Kjeldsen}, H. and {Bedding}, T.~R.},
    title = "{Amplitudes of solar-like oscillations: a new scaling relation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1104.1659},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, stars: oscillations, stars: general},
     year = 2011,
    month = may,
   volume = 529,
      eid = {L8},
    pages = {L8},
      doi = {10.1051/0004-6361/201116789},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...529L...8K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{brown91,
   author = {{Brown}, T.~M. and {Gilliland}, R.~L. and {Noyes}, R.~W. and 
    {Ramsey}, L.~W.},
    title = "{Detection of possible p-mode oscillations on Procyon}",
  journal = {\apj},
 keywords = {F STARS, LATE STARS, STELLAR OSCILLATIONS, SUBGIANT STARS, CHARGE COUPLED DEVICES, DOPPLER EFFECT, POWER SPECTRA, STELLAR LUMINOSITY, STELLAR TEMPERATURE},
     year = 1991,
    month = feb,
   volume = 368,
    pages = {599-609},
      doi = {10.1086/169725},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...368..599B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{verner11,
   author = {{Verner}, G.~A. and {Elsworth}, Y. and {Chaplin}, W.~J. and 
    {Campante}, T.~L. and {Corsaro}, E. and {Gaulme}, P. and {Hekker}, S. and 
    {Huber}, D. and {Karoff}, C. and {Mathur}, S. and {Mosser}, B. and 
    {Appourchaux}, T. and {Ballot}, J. and {Bedding}, T.~R. and 
    {Bonanno}, A. and {Broomhall}, A.-M. and {Garc{\'{\i}}a}, R.~A. and 
    {Handberg}, R. and {New}, R. and {Stello}, D. and {R{\'e}gulo}, C. and 
    {Roxburgh}, I.~W. and {Salabert}, D. and {White}, T.~R. and 
    {Caldwell}, D.~A. and {Christiansen}, J.~L. and {Fanelli}, M.~N.
    },
    title = "{Global asteroseismic properties of solar-like oscillations observed by Kepler: a comparison of complementary analysis methods}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1105.0571},
 primaryClass = "astro-ph.SR",
 keywords = {stars: fundamental parameters, stars: interiors, stars: oscillations, stars: solar-type},
     year = 2011,
    month = aug,
   volume = 415,
    pages = {3539-3551},
      doi = {10.1111/j.1365-2966.2011.18968.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.415.3539V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bedding03,
   author = {{Bedding}, T.~R. and {Kjeldsen}, H.},
    title = "{Solar-like Oscillations}",
  journal = {\pasa},
   eprint = {arXiv:astro-ph/0305425},
 keywords = {stars: oscillations},
     year = 2003,
   volume = 20,
    pages = {203-212},
      doi = {10.1071/AS03025},
   adsurl = {http://adsabs.harvard.edu/abs/2003PASA...20..203B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1974MNRAS.167..475H,
   author = {{Hanbury Brown}, R. and {Davis}, J. and {Lake}, R.~J.~W. and 
	{Thompson}, R.~J.},
    title = "{The effects of limb darkening on measurements of angular size with an intensity interferometer}",
  journal = {\mnras},
     year = 1974,
    month = jun,
   volume = 167,
    pages = {475-484},
   adsurl = {http://adsabs.harvard.edu/abs/1974MNRAS.167..475H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hanbury67,
   author = {{Hanbury Brown}, R. and {Davis}, J. and {Allen}, L.~R. and {Rome}, J.~M.
	},
    title = "{The stellar interferometer at Narrabri Observatory-II. The angular diameters of 15 stars}",
  journal = {\mnras},
     year = 1967,
   volume = 137,
    pages = {393},
   adsurl = {http://adsabs.harvard.edu/abs/1967MNRAS.137..393H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1968SJNA....5..506S,
   author = {{Strang}, G.},
    title = "{On the Construction and Comparison of Difference Schemes}",
  journal = {SIAM Journal on Numerical Analysis},
     year = 1968,
    month = sep,
   volume = 5,
    pages = {506-517},
      doi = {10.1137/0705041},
   adsurl = {http://adsabs.harvard.edu/abs/1968SJNA....5..506S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...515A..12C,
   author = {{Chiavassa}, A. and {Haubois}, X. and {Young}, J.~S. and {Plez}, B. and 
	{Josselin}, E. and {Perrin}, G. and {Freytag}, B.},
    title = "{Radiative hydrodynamics simulations of red supergiant stars. II. Simulations of convection on Betelgeuse match interferometric observations}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1003.1407},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: Betelgeuse, stars: atmospheres, hydrodynamics, radiative transfer, techniques: interferometric},
     year = 2010,
    month = jun,
   volume = 515,
    pages = {A12 },
      doi = {10.1051/0004-6361/200913907},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...515A..12C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2006sf2a.conf..455C,
   author = {{Chiavassa}, A. and {Plez}, B. and {Josselin}, E. and {Freytag}, B.
	},
    title = "{Line formation in 3D radiation hydrodynamics simulations of red supergiants}",
booktitle = {SF2A-2006: Semaine de l'Astrophysique Francaise},
     year = 2006,
   editor = "{D.~Barret, F.~Casoli, G.~Lagache, A.~Lecavelier, \& L.~Pagani
	}",
    month = jun,
    pages = {455},
   adsurl = {http://adsabs.harvard.edu/abs/2006sf2a.conf..455C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2010arXiv1011.2092V,
   author = {{Van Eck}, S. and {Neyskens}, P. and {Plez}, B. and {Jorissen}, A. and 
	{Edvardsson}, B. and {Eriksson}, K. and {Gustafsson}, B. and 
	{Jorgensen}, {U.-G.} and {Nordlund}, A.},
    title = "{A grid of MARCS model atmospheres for S stars}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1011.2092},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics},
     year = 2010,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1011.2092V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2005ApJ...628..973L,
   author = {{Levesque}, E.~M. and {Massey}, P. and {Olsen}, K.~A.~G. and
        {Plez}, B. and {Josselin}, E. and {Maeder}, A. and {Meynet}, G.
        },
    title = "{The Effective Temperature Scale of Galactic Red Supergiants: Cool, but Not As Cool As We Thought}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0504337},
 keywords = {ISM: Dust, Extinction, Stars: Atmospheres, Stars: Fundamental Parameters, Stars: Late-Type, Stars: Supergiants},
     year = 2005,
    month = aug,
   volume = 628,
    pages = {973-985},
      doi = {10.1086/430901},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005ApJ...628..973L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2006CoAst.147...76A,
   author = {{Asplund}, M. and {Grevesse}, N. and {Sauval}, A.~J.},
    title = "{The new solar abundances - Part I: the observations}",
  journal = {Communications in Asteroseismology},
     year = 2006,
    month = jan,
   volume = 147,
    pages = {76-79},
   adsurl = {http://adsabs.harvard.edu/abs/2006CoAst.147...76A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2000A&A...359..755A,
   author = {{Asplund}, M.},
    title = "{Line formation in solar granulation. III. The photospheric Si and meteoritic Fe abundances}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0005322},
 keywords = {CONVECTION, HYDRODYNAMICS, LINE: FORMATION, SUN: ABUNDANCES, SUN: GRANULATION, SUN: PHOTOSPHERE},
     year = 2000,
    month = jul,
   volume = 359,
    pages = {755-758},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...359..755A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2007A&A...469..687C,
   author = {{Collet}, R. and {Asplund}, M. and {Trampedach}, R.},
    title = "{Three-dimensional hydrodynamical simulations of surface convection in red giant stars. Impact on spectral line formation and abundance analysis}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0703652},
 keywords = {convection, hydrodynamics, line: formation, stars: abundances, stars: late-type, stars: atmospheres},
     year = 2007,
    month = jul,
   volume = 469,
    pages = {687-706},
      doi = {10.1051/0004-6361:20066321},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..687C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INBOOK{2000eaa..bookE1996N,
   author = {{Nordlund}, {\AA}. and {Murdin}, P.},
    title = "{Solar Interior: Convection Theory}",
 keywords = {Sun, Solar Interior},
booktitle = {Encyclopedia of Astronomy and Astrophysics},
     year = 2000,
    month = nov,
   editor = "{Murdin, P.}",
      doi = {10.1888/0333750888/1996},
   adsurl = {http://adsabs.harvard.edu/abs/2000eaa..bookE1996N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992A&A...256..551P,
   author = {{Plez}, B. and {Brett}, J.~M. and {Nordlund}, A.},
    title = "{Spherical opacity sampling model atmospheres for M-giants. I - Techniques, data and discussion}",
  journal = {\aap},
 keywords = {GIANT STARS, M STARS, OPACITY, STELLAR ATMOSPHERES, STELLAR MODELS, ASTRONOMICAL SPECTROSCOPY, COMPUTERIZED SIMULATION, RADIATION PRESSURE, RADIATIVE TRANSFER, SUPERGIANT STARS},
     year = 1992,
    month = mar,
   volume = 256,
    pages = {551-571},
   adsurl = {http://adsabs.harvard.edu/abs/1992A%26A...256..551P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MHD,
   author = {{Mihalas}, D. and {Dappen}, W. and {Hummer}, D.~G.},
    title = "{The equation of state for stellar envelopes. II - Algorithm and
selected results}",
  journal = {\apj},
 keywords = {CHARGED PARTICLES, COMPUTATIONAL ASTROPHYSICS, EQUATIONS OF STATE,
STELLAR ATMOSPHERES, STELLAR ENVELOPES, ALGORITHMS, COSMIC PLASMA, COULOMB
COLLISIONS, FREE ENERGY, PERTURBATION THEORY},
     year = 1988,
    month = aug,
   volume = 331,
    pages = {815-825},
      doi = {10.1086/166601},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...331..815M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{asplund09,
   author = {{Asplund}, M. and {Grevesse}, N. and {Sauval}, A.~J. and {Scott}, P.
        },
    title = "{The Chemical Composition of the Sun}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0909.0948},
 primaryClass = "astro-ph.SR",
     year = 2009,
    month = sep,
   volume = 47,
    pages = {481-522},
      doi = {10.1146/annurev.astro.46.060407.145222},
   adsurl = {http://adsabs.harvard.edu/abs/2009ARA%26A..47..481A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{stein98,
   author = {{Stein}, R.~F. and {Nordlund}, \AA.},
    title = "{Simulations of Solar Granulation. I. General Properties}",
  journal = {\apj},
 keywords = {METHODS: NUMERICAL, CONVECTION, SUN: GRANULATION, HYDRODYNAMICS, SUN:
INTERIOR},
     year = 1998,
    month = may,
   volume = 499,
    pages = {914-+},
      doi = {10.1086/305678},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...499..914S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2008A&A...486..951G,
   author = {{Gustafsson}, B. and {Edvardsson}, B. and {Eriksson}, K. and 
	{J{\o}rgensen}, U.~G. and {Nordlund}, {\AA}. and {Plez}, B.},
    title = "{A grid of MARCS model atmospheres for late-type stars. I. Methods and general properties}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0805.0554},
 keywords = {stars: atmospheres, Sun: abundances, stars: fundamental parameters, stars: general, stars: late-type, stars: supergiants},
     year = 2008,
    month = aug,
   volume = 486,
    pages = {951-970},
      doi = {10.1051/0004-6361:200809724},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...486..951G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004A&A...421..741V,
   author = {{V{\"o}gler}, A. and {Bruls}, J.~H.~M.~J. and {Sch{\"u}ssler}, M.
	},
    title = "{Approximations for non-grey radiative transfer in numerical simulations of the solar photosphere}",
  journal = {\aap},
 keywords = {Sun: photosphere, radiative transfer, methods: numerical},
     year = 2004,
    month = jul,
   volume = 421,
    pages = {741-754},
      doi = {10.1051/0004-6361:20047043},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...421..741V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997ApJ...483..390H,
   author = {{Hauschildt}, P.~H. and {Baron}, E. and {Allard}, F.},
    title = "{Parallel Implementation of the PHOENIX Generalized Stellar Atmosphere Program}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9607087},
 keywords = {METHODS: NUMERICAL, RADIATIVE TRANSFER, STARS: ATMOSPHERES},
     year = 1997,
    month = jul,
   volume = 483,
    pages = {390- },
      doi = {10.1086/304233},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...483..390H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992ApJ...397..717I,
   author = {{Iglesias}, C.~A. and {Rogers}, F.~J. and {Wilson}, B.~G.},
    title = "{Spin-orbit interaction effects on the Rosseland mean opacity}",
  journal = {\apj},
 keywords = {OPACITY, SPIN-ORBIT INTERACTIONS, STELLAR COMPOSITION, STELLAR INTERIORS, STELLAR MODELS, ABSORPTION SPECTRA, ABUNDANCE, EMISSION SPECTRA, METALLICITY},
     year = 1992,
    month = oct,
   volume = 397,
    pages = {717-728},
      doi = {10.1086/171827},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...397..717I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002AN....323..213F,
   author = {{Freytag}, B. and {Steffen}, M. and {Dorch}, B.},
    title = "{Spots on the surface of Betelgeuse --  Results from new 3D stellar convection models}",
  journal = {Astronomische Nachrichten},
 keywords = {methods: numerical, stars: individual (Betelgeuse), stars: spots, supergiants},
     year = 2002,
    month = jul,
   volume = 323,
    pages = {213-219},
      doi = {10.1002/1521-3994(200208)323:3/4<213::AID-ASNA213>3.0.CO;2-H},
   adsurl = {http://adsabs.harvard.edu/abs/2002AN....323..213F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986AnRFM..18..337R,
   author = {{Roe}, P.~L.},
    title = "{Characteristic-based schemes for the Euler equations}",
  journal = {Annual Review of Fluid Mechanics},
 keywords = {COMPUTATIONAL FLUID DYNAMICS, COMPUTERIZED SIMULATION, EULER EQUATIONS OF MOTION, METHOD OF CHARACTERISTICS, BOUNDARY VALUE PROBLEMS, CAUCHY PROBLEM, COMPUTATIONAL GRIDS, LINEAR EQUATIONS, SHOCK WAVE PROPAGATION},
     year = 1986,
   volume = 18,
    pages = {337-365},
      doi = {10.1146/annurev.fl.18.010186.002005},
   adsurl = {http://adsabs.harvard.edu/abs/1986AnRFM..18..337R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994IJNMF..18..555Q,
   author = {{Quirk}, J.~J.},
    title = "{A contribution to the great Riemann solver debate}",
  journal = {International Journal for Numerical Methods in Fluids},
     year = 1994,
    month = mar,
   volume = 18,
    pages = {555-574},
      doi = {10.1002/fld.1650180603},
   adsurl = {http://adsabs.harvard.edu/abs/1994IJNMF..18..555Q},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004A&A...414.1121W,
   author = {{Wedemeyer}, S. and {Freytag}, B. and {Steffen}, M. and {Ludwig}, {H.-G.} and 
	{Holweger}, H.},
    title = "{Numerical simulation of the three-dimensional structure and dynamics of the non-magnetic solar chromosphere}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0311273},
 keywords = {Sun: chromosphere, hydrodynamics, radiative transfer},
     year = 2004,
    month = feb,
   volume = 414,
    pages = {1121-1137},
      doi = {10.1051/0004-6361:20031682},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...414.1121W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...506.1351C,
   author = {{Chiavassa}, A. and {Plez}, B. and {Josselin}, E. and {Freytag}, B.
	},
    title = "{Radiative hydrodynamics simulations of red supergiant stars. I. interpretation of interferometric observations}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0907.1860},
 primaryClass = "astro-ph.SR",
 keywords = {stars: supergiants, stars: atmospheres, hydrodynamics, radiative transfer, techniques: interferometric},
     year = 2009,
    month = nov,
   volume = 506,
    pages = {1351-1365},
      doi = {10.1051/0004-6361/200911780},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...506.1351C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gray81,
   author = {{Gray}, D.~F.},
    title = "{Asymmetries in the spectral lines of Procyon}",
  journal = {\apj},
 keywords = {ASTRONOMICAL SPECTROSCOPY, LINE SHAPE, SPECTRAL LINE WIDTH, STELLAR SPECTRA, ASYMMETRY, CALCIUM, SOLAR SPECTRA, STELLAR SPECTROPHOTOMETRY},
     year = 1981,
    month = dec,
   volume = 251,
    pages = {583},
      doi = {10.1086/159501},
   adsurl = {http://adsabs.harvard.edu/abs/1981ApJ...251..583G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013arXiv1311.0329L,
   author = {{Lopez}, E.~D. and {Fortney}, J.~J.},
    title = "{Understanding the Mass-Radius Relation for Sub-Neptunes: Radius as a Proxy for Composition}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1311.0329},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics},
     year = 2013,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1311.0329L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dravins87,
   author = {{Dravins}, D.},
    title = "{Stellar Granulation - Part Two - Stellar Photospheric Line Asymmetries}",
  journal = {\aap},
     year = 1987,
    month = jan,
   volume = 172,
    pages = {211},
   adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...172..211D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1990A&A...228..155N,
   author = {{Nordlund}, A. and {Dravins}, D.},
    title = "{Stellar granulation. III - Hydrodynamic model atmospheres. IV - Line formation in inhomogeneous stellar photospheres. V - Synthetic spectral lines in disk-integrated starlight}",
  journal = {\aap},
 keywords = {ASTRONOMICAL MODELS, HYDRODYNAMICS, LATE STARS, SOLAR GRANULATION, STELLAR ATMOSPHERES, F STARS, G STARS, RADIATIVE TRANSFER, STELLAR MAGNETIC FIELDS, STELLAR TEMPERATURE, SUBGIANT STARS},
     year = 1990,
    month = feb,
   volume = 228,
    pages = {155-217},
   adsurl = {http://adsabs.harvard.edu/abs/1990A%26A...228..155N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1982A&A...107....1N,
   author = {{Nordlund}, A.},
    title = "{Numerical simulations of the solar granulation. I - Basic equations and methods}",
  journal = {\aap},
 keywords = {COMPUTERIZED SIMULATION, HYDRODYNAMIC EQUATIONS, RADIATIVE HEAT TRANSFER, SOLAR GRANULATION, SOLAR PHYSICS, CONTINUITY EQUATION, CONVECTION CURRENTS, EQUATIONS OF STATE, FOURIER SERIES, POISSON EQUATION, SOLAR ATMOSPHERE, SPECTRAL LINE WIDTH, SPLINE FUNCTIONS, STELLAR MODELS},
     year = 1982,
    month = mar,
   volume = 107,
    pages = {1-10},
   adsurl = {http://adsabs.harvard.edu/abs/1982A%26A...107....1N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...536..465S,
   author = {{Skartlien}, R.},
    title = "{A Multigroup Method for Radiation with Scattering in Three-Dimensional Hydrodynamic Simulations}",
  journal = {\apj},
 keywords = {Hydrodynamics, Methods: Numerical, Radiative Transfer, Sun: Atmosphere, Sun: Granulation},
     year = 2000,
    month = jun,
   volume = 536,
    pages = {465-480},
      doi = {10.1086/308934},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...536..465S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...541..468S,
   author = {{Skartlien}, R. and {Stein}, R.~F. and {Nordlund}, {\AA}.},
    title = "{Excitation of Chromospheric Wave Transients by Collapsing Granules}",
  journal = {\apj},
     year = 2000,
    month = sep,
   volume = 541,
    pages = {468-488},
      doi = {10.1086/309414},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...541..468S},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{2000SoPh..192...91S,
   author = {{Stein}, R.~F. and {Nordlund}, {\AA}.},
    title = "{Realistic Solar Convection Simulations}",
  journal = {\solphys},
     year = 2000,
    month = mar,
   volume = 192,
    pages = {91-108},
   adsurl = {http://adsabs.harvard.edu/abs/2000SoPh..192...91S},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{2000A&AS..146..267G,
   author = {{Gadun}, A.~S. and {Hanslmeier}, A. and {Pikalov}, K.~N. and 
	{Ploner}, S.~R.~O. and {Puschmann}, K.~G. and {Solanki}, S.~K.
	},
    title = "{Size-dependent properties of simulated 2-D solar granulation}",
  journal = {\aaps},
     year = 2000,
    month = oct,
   volume = 146,
    pages = {267-291},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26AS..146..267G},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}



@ARTICLE{2004A&A...421..755V,
   author = {{V{\"o}gler}, A.},
    title = "{Effects of non-grey radiative transfer on 3D simulations  of solar magneto-convection}",
  journal = {\aap},
     year = 2004,
    month = jul,
   volume = 421,
    pages = {755-762},
      doi = {10.1051/0004-6361:20047044},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...421..755V},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{1996A&A...313..497F,
   author = {{Freytag}, B. and {Ludwig}, H.-G. and {Steffen}, M.},
    title = "{Hydrodynamical models of stellar convection. The role of overshoot in DA white dwarfs, A-type stars, and the Sun.}",
  journal = {\aap},
     year = 1996,
    month = sep,
   volume = 313,
    pages = {497-516},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...313..497F},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJ...513L..49F,
   author = {{Freytag}, B. and {Salaris}, M.},
    title = "{Stellar Envelope Convection Calibrated by Radiation Hydrodynamics Simulations: Influence on Globular Cluster Isochrones}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/9901074},
     year = 1999,
    month = mar,
   volume = 513,
    pages = {L49-L52},
      doi = {10.1086/311912},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...513L..49F},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{1997ApJ...491L..47A,
   author = {{Asida}, S.~M. and {Tuchman}, Y.},
    title = "{Two-dimensional Simulation of Convection in a Red Giant Envelope}",
  journal = {\apjl},
     year = 1997,
    month = dec,
   volume = 491,
    pages = {L47 },
      doi = {10.1086/311055},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...491L..47A},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...528..896A,
   author = {{Asida}, S.~M.},
    title = "{Calibrating the Mixing-Length Parameter for a Red Giant Envelope}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9907446},
     year = 2000,
    month = jan,
   volume = 528,
    pages = {896-906},
      doi = {10.1086/308211},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...528..896A},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...524A..93C,
   author = {{Chiavassa}, A. and {Collet}, R. and {Casagrande}, L. and {Asplund}, M.
	},
    title = "{Three-dimensional hydrodynamical simulations of red giant stars: semi-global models for interpreting interferometric observations}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1009.1745},
 primaryClass = "astro-ph.SR",
 keywords = {stars: horizontal-branch, stars: atmospheres, hydrodynamics, radiative transfer, techniques: interferometric, stars: individual: HD 214868},
     year = 2010,
    month = dec,
   volume = 524,
    pages = {A93 },
      doi = {10.1051/0004-6361/201015507},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...524A..93C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2009LRSP....6....2N,
   author = {{Nordlund}, {\AA}. and {Stein}, R.~F. and {Asplund}, M.},
    title = "{Solar Surface Convection}",
  journal = {Living Reviews in Solar Physics},
 keywords = {solar physics, convection, granulation, mesogranulation, supergranulation},
     year = 2009,
    month = apr,
   volume = 6,
    pages = {2- },
   adsurl = {http://adsabs.harvard.edu/abs/2009LRSP....6....2N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009MmSAI..80..719C,
   author = {{Collet}, R. and {Nordlund}, {\AA}. and {Asplund}, M. and {Hayek}, W. and 
	{Trampedach}, R.},
    title = "{Abundance analysis of the halo giant HD 122563 with three-dimensional model stellar atmospheres}",
  journal = {Memorie della Societa Astronomica Italiana},
archivePrefix = "arXiv",
   eprint = {0909.0690},
 keywords = {Convection, Hydrodynamics, Line: formation, Stars: abundances, Stars: atmospheres, Stars: late-type, Stars: individual: HD122563},
     year = 2009,
   volume = 80,
    pages = {719- },
   adsurl = {http://adsabs.harvard.edu/abs/2009MmSAI..80..719C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1982A&A...107....1N,
   author = {{Nordlund}, A.},
    title = "{Numerical simulations of the solar granulation. I - Basic equations and methods}",
  journal = {\aap},
 keywords = {COMPUTERIZED SIMULATION, HYDRODYNAMIC EQUATIONS, RADIATIVE HEAT TRANSFER, SOLAR GRANULATION, SOLAR PHYSICS, CONTINUITY EQUATION, CONVECTION CURRENTS, EQUATIONS OF STATE, FOURIER SERIES, POISSON EQUATION, SOLAR ATMOSPHERE, SPECTRAL LINE WIDTH, SPLINE FUNCTIONS, STELLAR MODELS},
     year = 1982,
    month = mar,
   volume = 107,
    pages = {1-10},
   adsurl = {http://adsabs.harvard.edu/abs/1982A%26A...107....1N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994A&A...284..105L,
   author = {{Ludwig}, {H.-G.} and {Jordan}, S. and {Steffen}, M.},
    title = "{Numerical simulations of convection at the surface of a ZZ Ceti white dwarf}",
  journal = {\aap},
 keywords = {COMPUTERIZED SIMULATION, CONVECTIVE FLOW, NUMERICAL INTEGRATION, STELLAR ATMOSPHERES, STELLAR MODELS, VARIABLE STARS, WHITE DWARF STARS, EQUATIONS OF STATE, HYDRODYNAMICS, MIXING LENGTH FLOW THEORY, STELLAR TEMPERATURE},
     year = 1994,
    month = apr,
   volume = 284,
    pages = {105-117},
   adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...284..105L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2010A&A...515A..12C,
   author = {{Chiavassa}, A. and {Haubois}, X. and {Young}, J.~S. and {Plez}, B. and 
	{Josselin}, E. and {Perrin}, G. and {Freytag}, B.},
    title = "{Radiative hydrodynamics simulations of red supergiant stars. II. Simulations of convection on Betelgeuse match interferometric observations}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1003.1407},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: Betelgeuse, stars: atmospheres, hydrodynamics, radiative transfer, techniques: interferometric},
     year = 2010,
    month = jun,
   volume = 515,
    pages = {A12 },
      doi = {10.1051/0004-6361/200913907},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...515A..12C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
